Beating Adversarial Low-Rank MDPs with Unknown Transition and Bandit Feedback

We consider regret minimization in low-rank MDPs with fixed transition and adversarial losses. Previous work has investigated this problem under either full-information loss feedback with unknown transitions (Zhao et al., 2024), or bandit loss feedback with known transition (Foster et al., 2022). First, we improve the $poly(d, A, H)T^{5/6}$ regret bound of Zhao et al. (2024) to $poly(d, A, H)T^{2/3}$ for the full-information unknown transition setting, where d is the rank of the transitions, A is the number of actions, H is the horizon length, and T is the number of episodes. Next, we initiate the study on the setting with bandit loss feedback and unknown transitions. Assuming that the loss has a linear structure, we propose both model based and model free algorithms achieving $poly(d, A, H)T^{2/3}$ regret, though they are computationally inefficient. We also propose oracle-efficient model-free algorithms with $poly(d, A, H)T^{4/5}$ regret. We show that the linear structure is necessary for the bandit case without structure on the reward function, the regret has to scale polynomially with the number of states. This is contrary to the full-information case (Zhao et al., 2024), where the regret can be independent of the number of states even for unstructured reward function.

==> adaptive_prelims.tex <==
In this section, we deal with an adaptive adversary under the assumption that we are given the loss feature $\phi^\loss$, which may be different than the low-rank MDP feature $\phi^\star$.

\begin{assumption}[Loss Representation]
    \label{assm:linearloss}
    There is a (known) feature map $\phi^\loss$ satisfying \[\sup_{h\in[H],(x,a)\in \cX\times \cA}\|\phi^\loss_h(x,a)\|\leq 1\] and such that for any round $h\in[H]$, $t\in[T]$, and history $\cH\indd{t-1}=(x_{1:H}\indd{1:t-1},a_{1:H}\indd{1:t-1})$, the loss function $\ell_{h}(\cdot,\cdot;\cH\indd{t-1})$ satisfies:
    \begin{align}
     \forall (x,a)\in \cX\times \cA,\quad   \ell_{h}(x,a;\cH\indd{t-1}) = \phi^\loss_h(x,a)^\top \g _{h}\indd{t}, \label{eq:linearloss}
    \end{align} 
    for some $\g _{h}\indd{t}\in \bbB_d(1)$.
    \end{assumption}
\paragraph{Loss notation for adaptive adversary.}
\begin{itemize}
\item For round $t\in[T]$, denote $\cH\indd{t-1}\coloneqq (x_{1:H}\indd{t-1}, a_{1:H}\indd{t-1})$ the history of state-action pairs.
\item We assume that the loss at round $t$ is solely a function of the history and the current state-action pair;
\[\ell^t_h(x,a)= \ell_h(x,a;\cH\indd{t-1}).\]
\item For any two feature maps $\phi,\psi:\cX\times \cA \rightarrow \reals^d$, we denote by $[\phi,\psi]: \cX \times\cA \rightarrow \reals^{2d}$ the vertical stacking of the two feature maps.
\item For any $h\in[H]$, $t\in[T]$, policy $\pi\in \Pi$, history $\cH\indd{t-1}=(x_{1:H}\indd{t-1},a_{1:H}\indd{t-1})$, we denote by $Q^\pi_h(\cdot, \cdot;\cH\indd{t-1})$ the state-action (a.k.a.~$Q$-function) at layer $h$ corresponging to rollout policy $\pi$; that is,
 \begin{align}
    Q^\pi_h(x,a;\cH\indd{t-1}) \coloneqq \E^{\pi}\left[ \sum_{s=h}^H \ell_s(\x_s,\a_s; \cH\indd{t-1}) \mid \x_h = x, \a_h =a\right].
 \end{align}
 \item For history $\cH\indd{t-1}\coloneqq (x_{1:H}\indd{1:t-1},a_{1:H}\indd{1:t-1})$, we define 
 \begin{align}
     L\indd{t}(\pi) \coloneqq  L(\pi;\cH\indd{t-1}) \coloneqq  \E[Q^{\pi}_1(\x_1,\a_1;\cH\indd{t-1})]=\E^{\pi}\left[ \sum_{h=1}^H \ell_h(\x_h,\a_h;\cH\indd{t-1})\right]. \label{eq:lossdef}
 \end{align}
  \item For any distribution $\rho\in \Delta(\Pi)$, we use the notation $L(\rho;\cH\indd{t-1})=\E_{\bpi\sim \rho}[L(\bpi;\cH\indd{t-1})]$.
\end{itemize}


\begin{lemma}
\label{lem:linearQ}
For $t\in [T]$, $h\in [H]$, and $\pi\in\Pi$, there exists $\thetabar_h\indd{t,\pi} \in \bbB_{2d}(H \sqrt{d})$ such that for all $(x,a)\in \cX\times \cA$ and history $\cH\indd{t-1}=(x_{1:H}\indd{1:t-1},a_{1:H}\indd{1:t-1})$,
\begin{align}
    Q^\pi_h(x,a;\cH\indd{t-1})= \phibar^\star_h(x,a)^\top \thetab\indd{t,\pi}_h, \quad \text{where} \quad \phibar^\star_h \coloneqq [\phi^\loss, \phistar]\in \reals^{2d}.  \label{eq:theQ}
\end{align}
\end{lemma}
\begin{proof}
    Fix $t\in [T]$, $h\in [H]$, and $\pi\in\Pi$.
By the low-rank MDP structure and the normalizing assumption on $\mu^\star_h$ in \cref{assm:normalizing}, there exists $w^{t,\pi}_{h+1}\in \bbB_d((H-s)\sqrt{d})$ such that for all $(x,a)\in \cX\times \cA$ and history $\cH\indd{t-1}=(x_{1:H}\indd{1:t-1},a_{1:H}\indd{1:t-1})$,
\begin{align}
    \E^\pi\left[\sum_{s=h+1}^H \ell_s(\x_s,\a_s;\cH\indd{t-1}) \mid \x_h = x, \a_h =a\right] = \phi^\star_h(x,a)^\top w^{t,\pi}_{h+1}. \label{eq:linearfor}
\end{align}
Now, with $\g \indd{t}_h$ as in \cref{assm:linearloss}, \eqref{eq:linearloss} and \eqref{eq:linearfor} implies that $\thetab^{t,\pi}_h \coloneqq [\g \indd{t}_h, w\indd{t,\pi}_{h+1}]\in \reals^{2d}$ (where $[\cdot, \cdot]$ denotes the vertical stacking of vectors) satisfies the desired property.
\end{proof}

==> checklist.tex <==

\newpage
\section*{NeurIPS Paper Checklist}

%%% BEGIN INSTRUCTIONS %%%
The checklist is designed to encourage best practices for responsible machine learning research, addressing issues of reproducibility, transparency, research ethics, and societal impact. Do not remove the checklist: {\bf The papers not including the checklist will be desk rejected.} The checklist should follow the references and follow the (optional) supplemental material.  The checklist does NOT count towards the page
limit. 

Please read the checklist guidelines carefully for information on how to answer these questions. For each question in the checklist:
\begin{itemize}
    \item You should answer \answerYes{}, \answerNo{}, or \answerNA{}.
    \item \answerNA{} means either that the question is Not Applicable for that particular paper or the relevant information is Not Available.
    \item Please provide a short (1–2 sentence) justification right after your answer (even for NA). 
   % \item {\bf The papers not including the checklist will be desk rejected.}
\end{itemize}

{\bf The checklist answers are an integral part of your paper submission.} They are visible to the reviewers, area chairs, senior area chairs, and ethics reviewers. You will be asked to also include it (after eventual revisions) with the final version of your paper, and its final version will be published with the paper.

The reviewers of your paper will be asked to use the checklist as one of the factors in their evaluation. While "\answerYes{}" is generally preferable to "\answerNo{}", it is perfectly acceptable to answer "\answerNo{}" provided a proper justification is given (e.g., "error bars are not reported because it would be too computationally expensive" or "we were unable to find the license for the dataset we used"). In general, answering "\answerNo{}" or "\answerNA{}" is not grounds for rejection. While the questions are phrased in a binary way, we acknowledge that the true answer is often more nuanced, so please just use your best judgment and write a justification to elaborate. All supporting evidence can appear either in the main paper or the supplemental material, provided in appendix. If you answer \answerYes{} to a question, in the justification please point to the section(s) where related material for the question can be found.

% IMPORTANT, please:
% \begin{itemize}
%     \item {\bf Delete this instruction block, but keep the section heading ``NeurIPS paper checklist"},
%     \item  {\bf Keep the checklist subsection headings, questions/answers and guidelines below.}
%     \item {\bf Do not modify the questions and only use the provided macros for your answers}.
% \end{itemize} 
 

%%% END INSTRUCTIONS %%%


\begin{enumerate}

\item {\bf Claims}
    \item[] Question: Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \item[] Answer: \answerYes{}. % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The main claims made in the abstract and introductio accurately reflect the paper's contributions and scope. The claims are validated by detailed proofs.
    % \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the abstract and introduction do not include the claims made in the paper.
        \item The abstract and/or introduction should clearly state the claims made, including the contributions made in the paper and important assumptions and limitations. A No or NA answer to this question will not be perceived well by the reviewers. 
        \item The claims made should match theoretical and experimental results, and reflect how much the results can be expected to generalize to other settings. 
        \item It is fine to include aspirational goals as motivation as long as it is clear that these goals are not attained by the paper. 
    \end{itemize}

\item {\bf Limitations}
    \item[] Question: Does the paper discuss the limitations of the work performed by the authors?
    \item[] Answer:  \answerYes{}. %\answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The paper discuss the limitations of the work in the discussion section.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper has no limitation while the answer No means that the paper has limitations, but those are not discussed in the paper. 
        \item The authors are encouraged to create a separate "Limitations" section in their paper.
        \item The paper should point out any strong assumptions and how robust the results are to violations of these assumptions (e.g., independence assumptions, noiseless settings, model well-specification, asymptotic approximations only holding locally). The authors should reflect on how these assumptions might be violated in practice and what the implications would be.
        \item The authors should reflect on the scope of the claims made, e.g., if the approach was only tested on a few datasets or with a few runs. In general, empirical results often depend on implicit assumptions, which should be articulated.
        \item The authors should reflect on the factors that influence the performance of the approach. For example, a facial recognition algorithm may perform poorly when image resolution is low or images are taken in low lighting. Or a speech-to-text system might not be used reliably to provide closed captions for online lectures because it fails to handle technical jargon.
        \item The authors should discuss the computational efficiency of the proposed algorithms and how they scale with dataset size.
        \item If applicable, the authors should discuss possible limitations of their approach to address problems of privacy and fairness.
        \item While the authors might fear that complete honesty about limitations might be used by reviewers as grounds for rejection, a worse outcome might be that reviewers discover limitations that aren't acknowledged in the paper. The authors should use their best judgment and recognize that individual actions in favor of transparency play an important role in developing norms that preserve the integrity of the community. Reviewers will be specifically instructed to not penalize honesty concerning limitations.
    \end{itemize}

\item {\bf Theory Assumptions and Proofs}
    \item[] Question: For each theoretical result, does the paper provide the full set of assumptions and a complete (and correct) proof?
    \item[] Answer:  \answerYes{}. %\answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The paper provides detailed assumptions and proofs.  %\justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include theoretical results. 
        \item All the theorems, formulas, and proofs in the paper should be numbered and cross-referenced.
        \item All assumptions should be clearly stated or referenced in the statement of any theorems.
        \item The proofs can either appear in the main paper or the supplemental material, but if they appear in the supplemental material, the authors are encouraged to provide a short proof sketch to provide intuition. 
        \item Inversely, any informal proof provided in the core of the paper should be complemented by formal proofs provided in appendix or supplemental material.
        \item Theorems and Lemmas that the proof relies upon should be properly referenced. 
    \end{itemize}

    \item {\bf Experimental Result Reproducibility}
    \item[] Question: Does the paper fully disclose all the information needed to reproduce the main experimental results of the paper to the extent that it affects the main claims and/or conclusions of the paper (regardless of whether the code and data are provided or not)?
    \item[] Answer: \answerNA{}.% \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: This is a theoretical paper. %\justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item If the paper includes experiments, a No answer to this question will not be perceived well by the reviewers: Making the paper reproducible is important, regardless of whether the code and data are provided or not.
        \item If the contribution is a dataset and/or model, the authors should describe the steps taken to make their results reproducible or verifiable. 
        \item Depending on the contribution, reproducibility can be accomplished in various ways. For example, if the contribution is a novel architecture, describing the architecture fully might suffice, or if the contribution is a specific model and empirical evaluation, it may be necessary to either make it possible for others to replicate the model with the same dataset, or provide access to the model. In general. releasing code and data is often one good way to accomplish this, but reproducibility can also be provided via detailed instructions for how to replicate the results, access to a hosted model (e.g., in the case of a large language model), releasing of a model checkpoint, or other means that are appropriate to the research performed.
        \item While NeurIPS does not require releasing code, the conference does require all submissions to provide some reasonable avenue for reproducibility, which may depend on the nature of the contribution. For example
        \begin{enumerate}
            \item If the contribution is primarily a new algorithm, the paper should make it clear how to reproduce that algorithm.
            \item If the contribution is primarily a new model architecture, the paper should describe the architecture clearly and fully.
            \item If the contribution is a new model (e.g., a large language model), then there should either be a way to access this model for reproducing the results or a way to reproduce the model (e.g., with an open-source dataset or instructions for how to construct the dataset).
            \item We recognize that reproducibility may be tricky in some cases, in which case authors are welcome to describe the particular way they provide for reproducibility. In the case of closed-source models, it may be that access to the model is limited in some way (e.g., to registered users), but it should be possible for other researchers to have some path to reproducing or verifying the results.
        \end{enumerate}
    \end{itemize}


\item {\bf Open access to data and code}
    \item[] Question: Does the paper provide open access to the data and code, with sufficient instructions to faithfully reproduce the main experimental results, as described in supplemental material?
    \item[] Answer: \answerNA{} %\answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: This paper does not include experiments.  %\justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that paper does not include experiments requiring code.
        \item Please see the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item While we encourage the release of code and data, we understand that this might not be possible, so “No” is an acceptable answer. Papers cannot be rejected simply for not including code, unless this is central to the contribution (e.g., for a new open-source benchmark).
        \item The instructions should contain the exact command and environment needed to run to reproduce the results. See the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item The authors should provide instructions on data access and preparation, including how to access the raw data, preprocessed data, intermediate data, and generated data, etc.
        \item The authors should provide scripts to reproduce all experimental results for the new proposed method and baselines. If only a subset of experiments are reproducible, they should state which ones are omitted from the script and why.
        \item At submission time, to preserve anonymity, the authors should release anonymized versions (if applicable).
        \item Providing as much information as possible in supplemental material (appended to the paper) is recommended, but including URLs to data and code is permitted.
    \end{itemize}


\item {\bf Experimental Setting/Details}
    \item[] Question: Does the paper specify all the training and test details (e.g., data splits, hyperparameters, how they were chosen, type of optimizer, etc.) necessary to understand the results?
    \item[] Answer: \answerNA{}. %\answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: This paper does not include experiments. %\justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The experimental setting should be presented in the core of the paper to a level of detail that is necessary to appreciate the results and make sense of them.
        \item The full details can be provided either with the code, in appendix, or as supplemental material.
    \end{itemize}

\item {\bf Experiment Statistical Significance}
    \item[] Question: Does the paper report error bars suitably and correctly defined or other appropriate information about the statistical significance of the experiments?
    \item[] Answer: \answerNA{}. %\answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: This paper does not include experiments. %\justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The authors should answer "Yes" if the results are accompanied by error bars, confidence intervals, or statistical significance tests, at least for the experiments that support the main claims of the paper.
        \item The factors of variability that the error bars are capturing should be clearly stated (for example, train/test split, initialization, random drawing of some parameter, or overall run with given experimental conditions).
        \item The method for calculating the error bars should be explained (closed form formula, call to a library function, bootstrap, etc.)
        \item The assumptions made should be given (e.g., Normally distributed errors).
        \item It should be clear whether the error bar is the standard deviation or the standard error of the mean.
        \item It is OK to report 1-sigma error bars, but one should state it. The authors should preferably report a 2-sigma error bar than state that they have a 96\% CI, if the hypothesis of Normality of errors is not verified.
        \item For asymmetric distributions, the authors should be careful not to show in tables or figures symmetric error bars that would yield results that are out of range (e.g. negative error rates).
        \item If error bars are reported in tables or plots, The authors should explain in the text how they were calculated and reference the corresponding figures or tables in the text.
    \end{itemize}

\item {\bf Experiments Compute Resources}
    \item[] Question: For each experiment, does the paper provide sufficient information on the computer resources (type of compute workers, memory, time of execution) needed to reproduce the experiments?
    \item[] Answer: \answerNA{}. %\answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: This paper does not include experiments. %\justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The paper should indicate the type of compute workers CPU or GPU, internal cluster, or cloud provider, including relevant memory and storage.
        \item The paper should provide the amount of compute required for each of the individual experimental runs as well as estimate the total compute. 
        \item The paper should disclose whether the full research project required more compute than the experiments reported in the paper (e.g., preliminary or failed experiments that didn't make it into the paper). 
    \end{itemize}
    
\item {\bf Code Of Ethics}
    \item[] Question: Does the research conducted in the paper conform, in every respect, with the NeurIPS Code of Ethics \url{https://neurips.cc/public/EthicsGuidelines}?
    \item[] Answer: \answerYes{}.%\answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The research conducted in the paper conforms, in every respect, with the NeurIPS Code of Ethics.
    % This is a theoretical work.  %\justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the authors have not reviewed the NeurIPS Code of Ethics.
        \item If the authors answer No, they should explain the special circumstances that require a deviation from the Code of Ethics.
        \item The authors should make sure to preserve anonymity (e.g., if there is a special consideration due to laws or regulations in their jurisdiction).
    \end{itemize}


\item {\bf Broader Impacts}
    \item[] Question: Does the paper discuss both potential positive societal impacts and negative societal impacts of the work performed?
    \item[] Answer: \answerNA{} %\answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: This is a theoretical work. There is no societal impact of the work performed.%\justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that there is no societal impact of the work performed.
        \item If the authors answer NA or No, they should explain why their work has no societal impact or why the paper does not address societal impact.
        \item Examples of negative societal impacts include potential malicious or unintended uses (e.g., disinformation, generating fake profiles, surveillance), fairness considerations (e.g., deployment of technologies that could make decisions that unfairly impact specific groups), privacy considerations, and security considerations.
        \item The conference expects that many papers will be foundational research and not tied to particular applications, let alone deployments. However, if there is a direct path to any negative applications, the authors should point it out. For example, it is legitimate to point out that an improvement in the quality of generative models could be used to generate deepfakes for disinformation. On the other hand, it is not needed to point out that a generic algorithm for optimizing neural networks could enable people to train models that generate Deepfakes faster.
        \item The authors should consider possible harms that could arise when the technology is being used as intended and functioning correctly, harms that could arise when the technology is being used as intended but gives incorrect results, and harms following from (intentional or unintentional) misuse of the technology.
        \item If there are negative societal impacts, the authors could also discuss possible mitigation strategies (e.g., gated release of models, providing defenses in addition to attacks, mechanisms for monitoring misuse, mechanisms to monitor how a system learns from feedback over time, improving the efficiency and accessibility of ML).
    \end{itemize}
    
\item {\bf Safeguards}
    \item[] Question: Does the paper describe safeguards that have been put in place for responsible release of data or models that have a high risk for misuse (e.g., pretrained language models, image generators, or scraped datasets)?
    \item[] Answer: \answerNA{}. %\answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The paper poses no such risks. % \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper poses no such risks.
        \item Released models that have a high risk for misuse or dual-use should be released with necessary safeguards to allow for controlled use of the model, for example by requiring that users adhere to usage guidelines or restrictions to access the model or implementing safety filters. 
        \item Datasets that have been scraped from the Internet could pose safety risks. The authors should describe how they avoided releasing unsafe images.
        \item We recognize that providing effective safeguards is challenging, and many papers do not require this, but we encourage authors to take this into account and make a best faith effort.
    \end{itemize}

\item {\bf Licenses for existing assets}
    \item[] Question: Are the creators or original owners of assets (e.g., code, data, models), used in the paper, properly credited and are the license and terms of use explicitly mentioned and properly respected?
    \item[] Answer: \answerNA. % \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification:  This paper does not use existing assets. %\justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not use existing assets.
        \item The authors should cite the original paper that produced the code package or dataset.
        \item The authors should state which version of the asset is used and, if possible, include a URL.
        \item The name of the license (e.g., CC-BY 4.0) should be included for each asset.
        \item For scraped data from a particular source (e.g., website), the copyright and terms of service of that source should be provided.
        \item If assets are released, the license, copyright information, and terms of use in the package should be provided. For popular datasets, \url{paperswithcode.com/datasets} has curated licenses for some datasets. Their licensing guide can help determine the license of a dataset.
        \item For existing datasets that are re-packaged, both the original license and the license of the derived asset (if it has changed) should be provided.
        \item If this information is not available online, the authors are encouraged to reach out to the asset's creators.
    \end{itemize}

\item {\bf New Assets}
    \item[] Question: Are new assets introduced in the paper well documented and is the documentation provided alongside the assets?
    \item[] Answer: \answerNA{}. % \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: This paper does not release new assets. %\justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not release new assets.
        \item Researchers should communicate the details of the dataset/code/model as part of their submissions via structured templates. This includes details about training, license, limitations, etc. 
        \item The paper should discuss whether and how consent was obtained from people whose asset is used.
        \item At submission time, remember to anonymize your assets (if applicable). You can either create an anonymized URL or include an anonymized zip file.
    \end{itemize}

\item {\bf Crowdsourcing and Research with Human Subjects}
    \item[] Question: For crowdsourcing experiments and research with human subjects, does the paper include the full text of instructions given to participants and screenshots, if applicable, as well as details about compensation (if any)? 
    \item[] Answer: \answerNA{}. %\answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: This paper does not involve crowdsourcing nor research with human subjects. %\justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Including this information in the supplemental material is fine, but if the main contribution of the paper involves human subjects, then as much detail as possible should be included in the main paper. 
        \item According to the NeurIPS Code of Ethics, workers involved in data collection, curation, or other labor should be paid at least the minimum wage in the country of the data collector. 
    \end{itemize}

\item {\bf Institutional Review Board (IRB) Approvals or Equivalent for Research with Human Subjects}
    \item[] Question: Does the paper describe potential risks incurred by study participants, whether such risks were disclosed to the subjects, and whether Institutional Review Board (IRB) approvals (or an equivalent approval/review based on the requirements of your country or institution) were obtained?
    \item[] Answer: \answerNA{}. %\answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: This paper does not involve crowdsourcing nor research with human subjects. %\justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Depending on the country in which research is conducted, IRB approval (or equivalent) may be required for any human subjects research. If you obtained IRB approval, you should clearly state this in the paper. 
        \item We recognize that the procedures for this may vary significantly between institutions and locations, and we expect authors to adhere to the NeurIPS Code of Ethics and the guidelines for their institution. 
        \item For initial submissions, do not include any information that would break anonymity (if applicable), such as the institution conducting the review.
    \end{itemize}

\end{enumerate}



==> macros.tex <==
\newcommand{\cP}{\mathcal{P}}
\newcommand{\E}{\mathbb{E}}
\renewcommand{\P}{\mathbb{P}}
\newcommand{\cA}{\mathcal{A}}
\newcommand{\cC}{\mathcal{C}}
\newcommand{\veps}{\varepsilon}
\newcommand{\pistar}{\pi^\star}
\newcommand{\reg}{\mathrm{reg}}
\newcommand{\Bhat}{\widehat{B}}
\newcommand{\bell}{\bm{\ell}}
\newcommand{\replearn}{\mathrm{replearn}}
\newcommand{\pibar}{\bar{\pi}}
\newcommand{\Qbar}{\widebar{Q}}
\newcommand{\wtilde}{\widetilde}
\newcommand{\what}{\widehat{w}}
\newcommand{\pihat}{\widehat{\pi}}
\newcommand{\x}{\bm{x}}
\renewcommand{\a}{\bm{a}}
\newcommand{\phistar}{\phi^\star}
\newcommand{\dd}{\mathrm{d}}
\newcommand{\rep}{\mathrm{rep}}
\newcommand{\phirl}{\phihat^{\rl}}
\newcommand{\Qhat}{\widehat{Q}}
\newcommand{\ind}[1]{^{(#1)}}
\newcommand{\mustar}{\mu^\star}
\newcommand{\nn}{\nonumber}
\newcommand{\phihat}{\hat{\phi}}
\newcommand{\cX}{\mathcal{X}}
\newcommand{\cE}{\mathcal{E}}
\newcommand{\cG}{\mathcal{G}}
\newcommand{\cY}{\mathcal{Y}}
\newcommand{\cQ}{\mathcal{Q}}
\newcommand{\y}{\bm{y}}
%\newcommand{\bbB}{\bbB}
\newcommand{\bbB}{\mathbb{B}}
\newcommand{\reals}{\mathbb{R}}
\newcommand{\nreg}{N_\mathrm{reg}}
\newcommand{\cD}{\mathcal{D}}
\newcommand{\Sigmahat}{\widehat{\Sigma}}
\newcommand{\gen}{\mathrm{gen}}
\DeclareMathOperator*{\argmin}{argmin}
\newcommand{\unif}{\texttt{unif}}
\newcommand{\ldotst}{%
	\mathinner{{\ldotp}{\ldotp}}%
}
\newcommand{\cF}{\mathcal{F}}
\newcommand{\cH}{\mathcal{H}}
\newcommand{\fhat}{\hat{f}}
\newcommand{\vepsstatval}{c \cdot \frac{d\log(N_\reg K H/\delta)}{N_\reg}}
\newcommand{\vepsregval}{\frac{5H^3d^2\log(2 K H^2 d |\Phi| /\delta)}{N_\reg}}
\newcommand{\vepsregvalB}{\frac{37H^2d^2\beta^2\log(6 K H^2 d|\Phi| \delta^{-1} \gamma^{-1})}{N_\reg}}
\newcommand{\stat}{\mathrm{stat}}
\newcommand{\cov}{\mathrm{cov}}
\newcommand{\indd}[1]{^{#1}}
\newcommand{\cL}{\mathcal{L}}
\newcommand{\cI}{\mathcal{I}}
\newcommand{\bpi}{\bm{\pi}}
\newcommand{\cU}{\mathcal{U}}
\renewcommand{\u}{\bm{u}}
\newcommand{\z}{\bm{z}}
\newcommand{\bcH}{\bm{\cH}}
\newcommand{\thetahat}{\hat\theta}
\newcommand{\spanner}{\mathrm{span}}
\newcommand{\bzeta}{\bm{\zeta}}
\newcommand{\bh}{\bm{h}}
\newcommand{\est}{\texttt{LinEst}}
\newcommand{\psdp}{\texttt{PSDP}}
\newcommand{\estmat}{\texttt{EstMat}}
\newcommand{\veceval}{\texttt{EstVec}}
\newcommand{\rspanner}{\texttt{RobustSpanner}}
\newcommand{\apx}{\texttt{LinOpt}}
\newcommand{\btheta}{\bm{\theta}}
\newcommand{\bvartheta}{\tilde{\btheta}}
\newcommand{\Trepval}{\frac{A H \log(|\Phi|/\delta)}{\alpha \veps^2}}
\newcommand{\Tspanval}{\frac{A \log(d H|\Phi|\veps^{-1} \delta^{-1} )}{\alpha \veps^2}}
\newcommand{\Trepvalf}{\alpha^{-1}\veps^{-2} A H \log(|\Phi|/\delta)}
\newcommand{\Tspanvalf}{\alpha^{-2} \veps^{-2} A \log(d H|\Phi|\veps^{-1} \delta^{-1} )}
\newcommand{\Tcovval}{\veps^{-2}A d^{13} H^6 \log(\Phi/\delta)}
\newcommand{\loss}{\mathrm{loss}}
\newcommand{\freed}{\mathrm{freed}}
\newcommand{\phib}{\bar{\phi}}
\newcommand{\phibar}{\bar{\phi}}
\newcommand{\thetab}{\bar{\theta}}
\newcommand{\ww}{w}
\newcommand{\g}{g}
\newcommand{\varthetab}{\bm{\vartheta}}
\newcommand{\bvthetab}{\bar{\varthetab}}
\newcommand{\thetabar}{\bar{\theta}}


==> neurips/Introduction.tex <==
\section{Introduction}
%Over the past few years, reinforcement learning (RL) has sparked revolutions in various application areas, including game-playing~\citep{mnih2015human, silver2016mastering}, robotics~\citep{kober2013reinforcement, kalashnikov2018scalable} and fine-tuning large language models~\citep{ouyang2022training}. The empirical success of reinforcement learning has motivated researchers to explore its theoretical foundations. A central problem in reinforcement learning theory is identifying provably learnable settings with minimal assumptions. In stochastic environments, existing works have proposed various general classes that ensure learnability~\citep{jiang2017contextual,  jin2021bellman, du2021bilinear, foster2021statistical, zhong2022gec, chen2022statistical, chen2022unified, xie2022role, foster2023tight, foster2024model}. Remarkably, recent works~\citep{foster2021statistical, foster2023tight, foster2024model} characterize the statistical complexity of interactive decision-making, providing both necessary and sufficient condition for sample-efficient reinforcenemt learning in stochastic settings. 

We study online reinforcement learning (RL) in low-rank Markov Decision Processes (MDPs). Low-rank MDPs is a class of MDPs where the transition probability can be decomposed as an inner product between two low-dimensional features, i.e., $P(x'\mid x,a)=\phi^\star(x,a)^\top \mu^\star(x')$, where $P(x'\mid x,a)$ is the probability of transitioning to state $x'$ when the learner takes action $a$ on state $x$, and $\phi^\star$, $\mu^\star$ are two feature mappings. The ground truth features $\phi^\star$ and $\mu^\star$ are unknown to the learner. This setting has recently caught theoretical attention due to its simplicity and expressiveness \citep{ agarwal2020flambe, uehara2021representation, zhang2022making, cheng2023improved, modi2024model, zhang2022efficient, mhammedi2024efficient, huang2023reinforcement}.  In particular, since the learner does not know the features, it is necessary for the learner to perform \emph{feature learning} (or \emph{representation learning}) to approximate them. This allows low-rank MDPs to model the additional difficulty not present in traditional linear function approximation schemes where the features are given, such as in linear MDPs \citep{jin2020provably} and in linear mixture MDPs \citep{ayoub2020model}. Since feature learning is an indispensable part of modern deep RL
pipelines, low-rank MDP is a model that is closer to practice than traditional linear function approximation. 


Most prior theoretical work on low-rank MDPs focuses on reward-free learning; this is a setting where instead of focusing on a particular reward function, the goal is to learn a model for the transitions (or, in the model-free setting, a small set of policies with good state cover), that enables policy optimization for \emph{any} downstream reward functions. When these functions are chosen adversarially, most prior works have assumed full-information access to these functions \zm{cite works}. While this is a reasonable setup in some cases, in other applications, the learner can only obtain loss information from interactions with the environment, and only observes the loss on the state-actions that have been visited (i.e., bandit feedback). This introduces additional challenges to the learner. 

Furthermore, in many online learning scenarios, the loss function may change over time, reflecting the non-stationary nature of the environment or task switches \citep{padakandla2020reinforcement}. This could be modeled by the \emph{adversarial} MDP setting, where the loss function changes arbitrarily from one episode to the next, and the changes might even depend on the behavior of the learner. This setting is also extensively studied but mostly restricted to tabular MDPs \citep{rosenberg2019online, jin2020learning, shani2020optimistic, luo2021policy} or traditional linear function approximation schemes \jz{it's maybe not clear that this includes linear MDPs?}\citep{cai2020provably, luo2021policy, he2022near, zhao2022mixture, sherman2023improved, dai2023refined, liu2023towards}. The work by \cite{zhao2024learning} initiated the study on adversarial MDPs in low-rank MDPs, but their work is restricted to full-information loss feedback. 

When feature learning, bandit feedback, and adversarial losses are combined, the problem becomes highly challenging, and to the best of our knowledge their are no provably efficient algorithms to tackle this setting. In this work, we provide the first result for this combination. We hope that our result would bring new ideas to RL in practice, where all three elements are usually present simultaneously. 
We give four main results, targeting at either tighter regret (i.e., the performance gap between the optimal policy and the learner) or computational efficiency, summarized in \cref{tab:comparison}. Next, we briefly describe each of them. 

\begin{table}[t]
	\fontsize{8}{9}\selectfont
\caption{Comparison of Algorithms for the Adversarial Low-Rank MDP Setting}
\label{tab:comparison}
\centering
%\hspace*{-18pt}
\begin{tabular}{cccccc}
\toprule
\textbf{Algorithm} & \textbf{Algorithm type} & \textbf{Feedback} & \textbf{Regret} & \textbf{Efficiency} & \textbf{Note}\\ 
\midrule
\cite{zhao2024learning} & Model-based & Full-info & $T^{\nicefrac{5}{6}}$ & Oracle-efficient &Arbitrary loss \\ \midrule
\cref{alg:full-info} & Model-based & Full-info & $\sqrt{T}$ & Inefficient & Arbitrary loss  \\ 
\midrule
\cref{alg:low-rank bandit} & Model-based & Bandit & $T^{\nicefrac{2}{3}}$ & Inefficient & \makecell{Linear loss\\ Unknown loss feature}  \\ 
\midrule
\cref{alg:oraceleff} & Model-free & Bandit & $T^{\nicefrac{5}{6}}$ & Oracle-efficient & \makecell{Linear loss\\ Unknown loss feature}  \\  
\midrule
\makecell{\cref{alg:algorithm_name} \\ (For adaptive adversary)} & Model-free & Bandit & $T^{\nicefrac{5}{6}}$ & Oracle-efficient & \makecell{Linear loss \\ Known loss feature }\\ 
 \bottomrule
\end{tabular}

\end{table}



%Beyond stochastic environments, the more general adversarial settings consider loss functions that are changing over time, capturing the non-stationary nature of the real world, which is critical for complex robot learning tasks 
%\citep{padakandla2020reinforcement}. In constrast to the stochastic settings, the learnable instances in adversarial settings are far from fully understood, with results only derived for restrictive cases.  For adversarial reinforcement learning with known transition, \cite{foster2022complexity} shows it is as easy as stochastic settings. When transition is unknown, previous results are mainly derived for linear mixture MDPs~\citep{cai2020provably, he2022near, zhao2022mixture} or linear MDPs~\citep{luo2021policy,dai2023refined,sherman2023improved,kong2023improved,liu2023towards, sherman2023rate}, where the transition is assumed to have low-rank structure and the embedding feature for state-action pairs into the low-dimensional space is \emph{known}.  However, in real-world applications, it is difficult to have any prior knowledge on the feature maps, making representation learning necessary in reinforcememt learning \citep{bellemare2016unifying,pathak2017curiosity, tang2017exploration, oord2018representation, silver2018general, laskin2020curl, stooke2021decoupling, yang2021representation}. 

%Theoretical studies of representation learning for RL mainly focus on \emph{low-rank MDPs}, where the transition also has low-rank structure but the embedding feature is \emph{unknown}. Previous work have conducted extensive study for low-rank MDPs in stochatic setting with either model-based~\citep{ uehara2021representation, zhang2022making, cheng2023improved} or model-free approches~\cite{modi2024model, zhang2022efficient, mhammedi2024efficient}. However, efficent representation learning to handle adversarial low-rank MDPs remains largely unexplored. \cite{zhao2024learning} initialzes the study for this setting, but their algorithm requires the adversarial loss function is fully exposed to the learner and only get suboptimal $T^{\frac{5}{6}}$ regret. This motivates us to investigate whether it is possible to do better for representation learning with adversarial losses. 

%In our paper, we make significant progress in this direction. We not only improve the regret bound from $T^{\frac{5}{6}}$ to $\sqrt{T}$ with full infomation feedback, but also demonstrate that learning on low-rank MDPs with linear adversarial losses is even achievable for more challenging bandit feedback settings. (Add the necessarity for linear loss; I would just mention they are linear and discuss this later) For bandit feedback settings, we propose a model-based inefficient algorithm with $T^{\frac{2}{3}}$ regret and a model-free oracle-efficient algorithm with $T^{\frac{5}{6}}$ regret. 
%Since both the embedding features and loss function are unknown in bandit feedback settings, standard loss estimator is not applicable and we propose two new estimators to tackle this challenge. Our algorithms are summarized below.

\begin{itemize}[leftmargin=10pt]

\item \textbf{$\sqrt{T}$-regret model-based algorithm under full-information feedback (\cref{alg:full-info})}.  This algorithm is based on policy optimization \citep{luo2021policy} with a carefully designed exploration bonus that facilitates \emph{point-wise} uncertain quantification. %The exploration bonus is designed in a model-based manner using the width of a transition confidence set based on maximum likelihood estimation. We show that such a bonus leads to more efficient exploration, 
This improves over the $T^{\nicefrac{5}{6}}$ regret of \cite{zhao2024learning} in the same setting whose exploration bonus is based on \emph{global optimism}.  % to $\sqrt{T}$ under full information.

\item \textbf{$T^{\nicefrac{2}{3}}$-regret model-based algorithm under bandit feedback (\cref{alg:low-rank bandit})}. %This algorithm begins with a model-based initial exploration phase to learn an estimated transition and the corresponding features. In the subsequent episodes, we utilize 
This algorithm begins with an initial exploration phase to learn an estimated transition, and then runs exponential weights over policies for regret minimization in the second phase.  %For every episode, a behavior policy is drawn from the current policy distribution to collect data. 
For exponential weights, we use a novel loss estimator inspired by linear bandits while leveraging the structure of low-rank MDP. % The loss estimators also carefully leverage the low-rank structure to ensure its bias is only related to the estimated error for features, which can be effectively compensated by incorporating an exploration bonus into the exponential weights.



\item \textbf{$T^{\nicefrac{5}{6}}$-regret model-free oracle-efficient algorithm under bandit feedback (\cref{alg:oraceleff}). } This algorithm also starts with an exploration phase, where it calls \texttt{VoX} \cite{mhammedi2023efficient} to learn a policy cover; \texttt{VoX} is a model-free, reward-free exploration algorithm. After this initial exploratory phase, the algorithm operates in epochs; during epoch $k$, the algorithm commits to a fixed mixture of policies. This mixture consists of certain exploratory policies (based on the policy cover from the initial phase) and a policy computed using an online learning algorithm (similar to \cite{dai2023refined}) based on estimated $Q$-functions from previous epochs (these act as loss functions). %Mixing with eploratory policies is needed here to estimate the $Q$-functions that the online algorithm uses. 
\item \textbf{$T^{\nicefrac{5}{6}}$-\bf{adaptive} regret model-free oracle-efficient algorithm under bandit feedback (\cref{alg:algorithm_name}). } This algorithm deals with the much more challenging setting of an \emph{adaptive} adversary with bandit feedback. Here, we make the additional assumption that the loss feature, which may be different from the feature of the low-rank decomposition, is given. The algorithm is similar to the previous model-free algorithm with key differences outlined in \cref{sec:extension}.% after computing a policy cover, the algorithm calls $\texttt{RepLearn}$ to compute a feature map $\phi^\rep$. Then, for every $h\in[H]$, the algorithm computes a \emph{spanner}; a set of policies $\Psi^\spanner_h =\{\pi_{h,1},\dots,\pi_{h,d}\}$ that act as an approximate spanner for the set $\{\E^{\pi}[\phi^\rep_h(\x_h,\a_h)]:\pi \in \Pi\}\subseteq \reals^d$. These spanner policies are then used as the exploratory policies after the initial phase; we require these spanner policies instead of policies in the poly cover because the estimation of the $Q$-functions become much more challenging with an adaptive adversary. 
\end{itemize}

Our algorithms provide new insights on representation learning for RL and also broaden the scope for provably efficient reinforcement learning in adversarial settings.

We provide a more thorough related work review in \cref{app: related work}. 

==> neurips/Preliminaries.tex <==
\section{Preliminaries}
\label{sec:prelim}
We study the episodic online reinforcement learning setting with horizon $H$. We consider an MDP $\mathcal M=(\cX, \cA, P_{1:H}^\star)$, where
$\cX$ represents a countable (possibly infinite) state space\footnote{We assume that $\cX$ is
countable only to simplify the presentation. Our results can easily be extended to a continuous state space with an appropriate measure-theoretic
treatment (see e.g.~\cite{mhammedi2023efficient}).}, 
$\cA$ is a finite action space, and $P^\star_h: \cX \times \cA \rightarrow \Delta(\cX)$ denotes the transition kernel from layer $h$ to $h+1$. We assume that the initial state $x_1\in \cX$ is fixed for simplicity and without loss of generality.
For any policy $\pi:\cX \mapsto \Delta(\cA)$ and arbitrary set of transition kernels $\{P_h\}_{h\in[H]}$, we let $\P^{P,\pi}$ denote the law over $(\x_{1},\a_1,\dots,\x_H,\a_H)$ induced by the process of setting $\x_1 =x_1$, sampling $\a_1\sim \pi_1(\cdot \mid \x_1)$, then for $h=2,\dots, H$, $\x_{h}\sim P_{h-1}(\cdot \mid \x_{h-1},\a_{h-1})$ and $\a_h \sim \pi_h(\cdot\mid \x_h)$. We let $\E^{P,\pi}$ denote the corresponding expectations. Further, we let $d^{P,\pi}_h(x)\coloneqq \P^{P,\pi}[\x_h= x]$ denote the \emph{occupancy} of $x\in \cX$. We also let $d^{P,\pi}_h(x,a)\coloneqq \P^{P,\pi}[\x_h= x,\a_h=a]$. Further, we let $\E^{\pi}=\E^{P^\star,\pi}$, $\P^{\pi}=\P^{P^\star,\pi}$, and $d^{\pi}_h=d_h^{P^\star,\pi}$. 


%\zmdelete{We assume the state space $\cX$ is organized to have distinct, non-overlapping \textit{layers}, i.e., $\cX=\cX_1 \cup \cX_2 \cup \cdots \cup \cX_H$ where $\cX_{h}\cap \cX_{h'}=\varnothing$ for any $1\le h<h'\le H$ \zm{Do we need this?}, and transition is only possible from one layer to the next. The transition at layer $h$ is determined by $P_h^\star \colon \cX_h \times \cA\to \Delta(\cX_{h+1})$.  For simplicity, and without loss of generality, we assume $\cX_1=\{x_1\}$ as the fixed initial state for every episode. \zm{Do we need this?}}




% $P_h^\star \colon \cX\times \cA\to \Delta(\cX)$ is the transition kernal of step $h$. 





% We assume the state space $\cX$ is organized to have distinct, non-overlapping \textit{layers}, i.e., $\cX=\cX_1 \cup \cX_2 \cup \cdots \cup \cX_H$ where $\cX_{h}\cap \cX_{h'}=\varnothing$ for any $1\le h<h'\le H$, and transition is only possible from one layer to the next, that is, $P(x' \mid x,a) \neq 0$ only when $s \in \cX_h$ and $x' \in \cX_{h+1}$. For simplicity, and without loss of generality, we assume $\cX_1=\{x_1\}$ as the fixed initial state for every episode.

We consider a learner interacting with the MDP $\mathcal M$ for $T$ episodes with adversarial loss functions. Before the game starts, an oblivious adversary chooses the loss functions for all episodes $(\ell^t_{1:H}: \cX \times \cA \rightarrow  [0,1])_{t=1}^T$. For each episode $t \in [T]$, the learner starts at state $\x_{1}^t = x_1$, then for each step $h\in [H]$ within episode $t$, the learner observes state 
$\x_{h}^t\in\cX_h$, chooses an action $\a_h^t \in \cA$, then suffers loss $\ell_{h}^t(\x_{h}^t,\a_{h}^t)$. The state $\x_{h+1}^t$  at the next step is drawn from transition $P^\star_{h}(\cdot \mid \x_{h}^t,\a_{h}^t)$. We consider both full information and bandit feedback settings. For \textit{full information} setting, the learner could observe the loss function $\ell^t$ for every episode. On the other hand, for the \textit{bandit feedback} setting, the learner could only observe the losses $\ell^t_1(\x^t_1,\a^t_1), \dots, \ell^t_H(\x^t_H,\a^t_H)$ at the visited state-action pairs.


We let $\Pi\coloneqq \{\pi: \cX \rightarrow \cA\}$ denote the set of Markovian policies $\pi$. For policy $\pi\in \Pi$, loss $\ell$ and transition kernels $P_{1:H}$, we denote by $Q^{P,\pi}_h(\cdot,\cdot; \ell)$ the \emph{state-action} value function (a.k.a.~$Q$-function) at step $h\in[H]$ with respect to the transitions $P_{1:H}$ and loss $\ell$; that is
\begin{align}
\label{eq: Q-function}
Q^{P,\pi}_h(x,a; \ell) \coloneqq  \E^{P,\pi}\left[\sum_{s=h}^H \ell_s(\x^t_{s},\a^t_{s})  \mid \x_h=x, \a_h =a \right],
\end{align}
for all $(x,a)\in \cX\times \cA$. We let $V^{P,\pi}_h(x; \ell) \coloneqq \max_{a\in \cA} Q^{P,\pi}_h(x,a;\ell)$ be the corresponding \textit{state} value function at layer $h$. Further, we write $Q^{\pi}_h(\cdot,\cdot; \ell)\coloneqq Q^{P^\star,\pi}_h(\cdot,\cdot; \ell)$ and $V^{\pi}_h( \cdot;\ell)\coloneqq V^{P^\star,\pi}( \cdot;\ell)$.

For the first three algorithms (\cref{alg:full-info}--\cref{alg:oraceleff}), we aim to construct (possibly randomized) policies $\{\bpi^t\}_{t\in[T]}$ that ensure a sublinear \emph{pseudo-regret} with respect to the best-fixed policy; that is,
\begin{align}
\mathrm{Reg}_T \coloneqq  \min_{\pi\in \Pi}\mathrm{Reg}_T(\pi) \quad \text{where} \quad \mathrm{Reg}_T(\pi) \coloneqq \E\left [\sum_{t=1}^T V_1^{\bpi^t}(x_1; \ell^t) - \sum_{t=1}^T V_1^{\pi}(x_1; \ell^t)\right]. 
\end{align}

For the last algorithm (\cref{alg:algorithm_name}), we bound the standard \emph{regret} 
\begin{align*}
    \overline{\mathrm{Reg}}_T := \sum_{t=1}^T V_1^{\pi^t}(x_1; \ell^t) - \min_{\pi\in\Pi}\sum_{t=1}^T V_1^{\pi}(x_1; \ell^t) 
\end{align*}
with high probability. This allows it to handle adaptive adversary.  


Throughout, we will assume that the MDP $\cM$ is low-rank with \emph{unknown} feature maps $\phistar_h$ and $\mu^\star_h$.
\begin{assumption}[Low-Rank MDP]
\label{assm:normalizing}
    There exist (unknown) features maps $\phistar_{1:H}:\cX\times \cA\rightarrow \reals^d$ and $\mu^\star_{1:H}:\cX \rightarrow \reals^d$, such that for all $h\in[H-1]$ and $(x,a,x')\in \cX\times \cA\times \cX$:
\begin{align}
\P[\x_{h+1}=x'\mid \x_h=x,\a_{h}=a] =  \phistar_h(x,a)^\top \mu^\star_{h+1}(x'). \label{eq:lr}
\end{align}
   Furthermore, for all $h\in[H]$, the feature maps $\mu^\star_h$ and $\phistar_h$ are such that $\sup_{(x,a)\in \cX\times \cA}\|\phistar_h(x,a)\|\leq 1$ and  $\|\sum_{x\in \cX}g(x)\cdot \mu^\star_h(x)\|\leq \sqrt{d}$, for all $g:\cX\rightarrow [0,1]$.
\end{assumption}


 
\begin{comment}
\begin{definition}[Low-rank MDP]\label{def: low-rank MDP} In \textit{low-rank MDP}, for any layer $h \in [H]$, each state $x \in \cX_h$ and action $a\in \cA$ is associated with an (unknown) feature $\phi_h^\star(x,a)\in \mathbb R^d$ with $\| \phi_h^\star(s,a) \|_2\le 1$.
There exists an (unknown) mapping $\psi_{h} \colon \cX_{h+1} \to \mathbb{R}^d$ such that the transition can be expressed as
\begin{align*}
P_h^\star(x'\mid x,a) &= \langle \phi_h^\star(x,a),\psi_{h}(x')\rangle,\quad \forall (x,a,x')\in \cX_{h}\times \cA\times \cX_{h+1}.    \label{eq: P assumption}
\end{align*}
For any measurable function $g: \cX \to \mathbb{R}^d$ such that $\|g\|_{\infty} \le 1$, we have $\left\|\int \psi_h(x)g(x) dx\right\|_2 \le \sqrt{d}$ for all $h \in [H]$.
\end{definition}
\end{comment}

\paragraph{Loss function under bandit feedback.} 
For bandit feedback setting, we make the following additional linear assumption on the losses; in the sequel, we will argue that this is necessary to avoid a sample complexity scaling with the number of states. This linear loss assumption also appears in \cite{ren2022free,  zhang2022making} for stochastic low-rank MDPs. Note that for the full-information feedback setting, such an assumption is not required. 


\begin{assumption}[Loss Representation]
    \label{assm:linearlossweak}
   For any $t\in[T]$ and layer $h$, there is a vector $g_{h}\indd{t}\in \mathbb{B}_d(1)$ such that the loss $\ell^t_{h}(x,a)$ at round $t$ satisfies:
    \begin{align}
     \forall (x,a)\in \cX\times \cA,\quad   \ell^t_{h}(x,a) = \phi^\star_h(x,a)^\top g_{h}\indd{t}. \label{eq:linearlossweak}
    \end{align} 
    \end{assumption}
We note that there is no loss of generality in assuming that the losses are expressed using the same features $\phistar_{1:H}$ as the low-rank structure in \eqref{eq:lr}. This is because if the losses have different features, we can simply combine these features with the low-rank features, and redefine $\phistar$ accordingly. For the bulk of our results (and as stated in the prequel), we will assume that the losses $\{\ell^t_{h}(\cdot,\cdot)\}_{h\in[H],t\in[T]}$ (or equivalently $\{g_h\indd{t}\}_{h\in[H],t\in[T]}$ under \cref{assm:linearlossweak}) are chosen by an aversary before the start of the game (i.e.~oblvious adversary). In \cref{sec:adaptive}, we will present a model-free, oracle-efficient algorithm for an adaptive adversary. 

\paragraph{Function approximation.}
So far, \cref{assm:normalizing} and \cref{assm:linearlossweak} are in line with assumptions made in the linear MDP setting \citep{jin2020provably}. However, unlike in linear MDPs, we do not assume that the feature maps $\phistar_{1:H}$ are known. To facilitate representation learning and ultimately a sublinear regret, we need to make \emph{realizability} assumptions. In particular, in the model-free setting (\cref{sec:model-free} and  \cref{sec:adaptive}) we assume we have a function class $\Phi$ that contains the true features $\phistar_{1:H}$. In the model-based setting (\cref{sec:full-info} and \cref{sec:model-based bandit}), we additionally assume access to a function class $\Upsilon$
that contains the feature maps $\mu^\star_{1:H}$\footnote{The setting where we assume access to function classes that realize both $\phistar_{1:H}$ and $\mustar_{1:H}$ is called \emph{model-based} because it allows one to model the transition probabilities, thanks to the low-rank structure in \eqref{eq:lr}.}. We will formalize these assumptions in their corresponding sections in the sequel.

\paragraph{Other notation.}  For $\psi:\Pi \rightarrow \reals^d$, we define $\john(\psi, \Pi)$ as a distribution $\mu\in\Delta(\Pi)$ such that $\|\psi(\pi)\|_{G^{-1}}^2\leq d$ for all $\pi\in\Pi$, where $G=\sum_{\pi\in\Pi} \mu(\pi)\cdot \psi(\pi)\psi(\pi)^\top$. This is the standard John's exploration or $G$-optimal design, which always exists. 




==> neurips/Related-Work.tex <==
\section{Related Work} \label{app: related work}
\paragraph{Learning low-rank MDPs in the stochastic setting. }
In the absent of adversarial losses, several general learning frameworks have been developed for super classes of low-rank MDPs which offer tight sample complexity for either reward-based \citep{jiang2017contextual,  jin2021bellman, du2021bilinear, foster2021statistical, zhong2022gec} or reward-free \citep{chen2022statistical, chen2022unified, xie2022role} settings. However, these algorithms require solving non-convex optimization problems on non-convex version spaces, making them computationally inefficiency. Oracle-efficient algorithms for low-rank MDPs are first obtained by \cite{agarwal2020flambe} using a model-based approach, and the sample complexity bound has been largely improved in subsequent works \citep{ uehara2021representation, zhang2022making, cheng2023improved}. The model-based approach, however, necessitates the function class to accurately model the transition, which is a strong requirement. To relax it, \cite{modi2024model, zhang2022efficient} developed oracle-efficient model-free algorithms, but both of them require additional assumptions on the MDP structure. Recently, \cite{mhammedi2024efficient} proposed a satisfactory model-free algorithm that removes all these assumptions. Our work leverages their techniques to tackle the more challenging adversarial setting.
~\\


% \cite{ren2022free,  zhang2022making} also use linear loss assumption. It seems \cite{ren2022free} is the only work that is efficient and have efficient $\sqrt{T}$-regret (although Bayesian guarantee)?

\paragraph{Learning adversarial MDPs.} Learning adversarial tabular MDPs under bandit feedback and unknown transition has been extensively studied~\citep{rosenberg2019online, jin2020learning, lee2020bias, jin2021best, shani2020optimistic, chen2021finding, luo2021policy, dai2022follow, dann2023best}. This line of work has demonstrated not only $\sqrt{T}$ regret bounds but also several data-dependent bounds.

For adversarial MDPs with a large state space which necessitates the use of function approximation, if the transition is known, \cite{foster2022complexity} shows that adversarial setting is as easy as the stochastic setting even under general function approximation. For full-information loss feedback with unknown transition, $\sqrt{T}$ bound is derived for both linear mixture MDPs \citep{cai2020provably, he2022near} and linear MDPs \citep{sherman2023rate}. For more challenging low-rank MDPs with unknown features, the best result only achieves  $T^{\nicefrac{5}{6}}$ regret~\citep{zhao2024learning}.

For function approximation with bandit feedback and unknown transition, \cite{zhao2022mixture} provides $\sqrt{T}$ bound for linear mixture MDPs, but their regret 
has polynomial dependence on the size of the state space due to the lack of structure on the loss function. For linear MDPs, a series of recent work has made significant progress in improving the regret bound~\citep{luo2021policy, dai2023refined, sherman2023improved, kong2023improved, liu2023towards}. The state-of-the-art result by \cite{liu2023towards} gives an  inefficient algorithm with $\sqrt{T}$ regret and an efficient algorithm with $T^{\nicefrac{3}{4}}$ regret. These regret bounds for linear MDPs do not depend on the state space size because of the linear loss assumption. We show that cross-state structure on the losses is necessary for low-rank MDPs with bandit feedback to achieve regret bound that do not scale with the number of states in \cref{sec:lower bound}.

==> neurips/checklist.tex <==

\newpage
\section*{NeurIPS Paper Checklist}

%%% BEGIN INSTRUCTIONS %%%
The checklist is designed to encourage best practices for responsible machine learning research, addressing issues of reproducibility, transparency, research ethics, and societal impact. Do not remove the checklist: {\bf The papers not including the checklist will be desk rejected.} The checklist should follow the references and follow the (optional) supplemental material.  The checklist does NOT count towards the page
limit. 

Please read the checklist guidelines carefully for information on how to answer these questions. For each question in the checklist:
\begin{itemize}
    \item You should answer \answerYes{}, \answerNo{}, or \answerNA{}.
    \item \answerNA{} means either that the question is Not Applicable for that particular paper or the relevant information is Not Available.
    \item Please provide a short (1–2 sentence) justification right after your answer (even for NA). 
   % \item {\bf The papers not including the checklist will be desk rejected.}
\end{itemize}

{\bf The checklist answers are an integral part of your paper submission.} They are visible to the reviewers, area chairs, senior area chairs, and ethics reviewers. You will be asked to also include it (after eventual revisions) with the final version of your paper, and its final version will be published with the paper.

The reviewers of your paper will be asked to use the checklist as one of the factors in their evaluation. While "\answerYes{}" is generally preferable to "\answerNo{}", it is perfectly acceptable to answer "\answerNo{}" provided a proper justification is given (e.g., "error bars are not reported because it would be too computationally expensive" or "we were unable to find the license for the dataset we used"). In general, answering "\answerNo{}" or "\answerNA{}" is not grounds for rejection. While the questions are phrased in a binary way, we acknowledge that the true answer is often more nuanced, so please just use your best judgment and write a justification to elaborate. All supporting evidence can appear either in the main paper or the supplemental material, provided in appendix. If you answer \answerYes{} to a question, in the justification please point to the section(s) where related material for the question can be found.

% IMPORTANT, please:
% \begin{itemize}
%     \item {\bf Delete this instruction block, but keep the section heading ``NeurIPS paper checklist"},
%     \item  {\bf Keep the checklist subsection headings, questions/answers and guidelines below.}
%     \item {\bf Do not modify the questions and only use the provided macros for your answers}.
% \end{itemize} 
 

%%% END INSTRUCTIONS %%%


\begin{enumerate}

\item {\bf Claims}
    \item[] Question: Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \item[] Answer: \answerYes{}. % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The main claims made in the abstract and introductio accurately reflect the paper's contributions and scope. The claims are validated by detailed proofs.
    % \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the abstract and introduction do not include the claims made in the paper.
        \item The abstract and/or introduction should clearly state the claims made, including the contributions made in the paper and important assumptions and limitations. A No or NA answer to this question will not be perceived well by the reviewers. 
        \item The claims made should match theoretical and experimental results, and reflect how much the results can be expected to generalize to other settings. 
        \item It is fine to include aspirational goals as motivation as long as it is clear that these goals are not attained by the paper. 
    \end{itemize}

\item {\bf Limitations}
    \item[] Question: Does the paper discuss the limitations of the work performed by the authors?
    \item[] Answer:  \answerYes{}. %\answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The paper discuss the limitations of the work in the discussion section.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper has no limitation while the answer No means that the paper has limitations, but those are not discussed in the paper. 
        \item The authors are encouraged to create a separate "Limitations" section in their paper.
        \item The paper should point out any strong assumptions and how robust the results are to violations of these assumptions (e.g., independence assumptions, noiseless settings, model well-specification, asymptotic approximations only holding locally). The authors should reflect on how these assumptions might be violated in practice and what the implications would be.
        \item The authors should reflect on the scope of the claims made, e.g., if the approach was only tested on a few datasets or with a few runs. In general, empirical results often depend on implicit assumptions, which should be articulated.
        \item The authors should reflect on the factors that influence the performance of the approach. For example, a facial recognition algorithm may perform poorly when image resolution is low or images are taken in low lighting. Or a speech-to-text system might not be used reliably to provide closed captions for online lectures because it fails to handle technical jargon.
        \item The authors should discuss the computational efficiency of the proposed algorithms and how they scale with dataset size.
        \item If applicable, the authors should discuss possible limitations of their approach to address problems of privacy and fairness.
        \item While the authors might fear that complete honesty about limitations might be used by reviewers as grounds for rejection, a worse outcome might be that reviewers discover limitations that aren't acknowledged in the paper. The authors should use their best judgment and recognize that individual actions in favor of transparency play an important role in developing norms that preserve the integrity of the community. Reviewers will be specifically instructed to not penalize honesty concerning limitations.
    \end{itemize}

\item {\bf Theory Assumptions and Proofs}
    \item[] Question: For each theoretical result, does the paper provide the full set of assumptions and a complete (and correct) proof?
    \item[] Answer:  \answerYes{}. %\answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The paper provides detailed assumptions and proofs.  %\justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include theoretical results. 
        \item All the theorems, formulas, and proofs in the paper should be numbered and cross-referenced.
        \item All assumptions should be clearly stated or referenced in the statement of any theorems.
        \item The proofs can either appear in the main paper or the supplemental material, but if they appear in the supplemental material, the authors are encouraged to provide a short proof sketch to provide intuition. 
        \item Inversely, any informal proof provided in the core of the paper should be complemented by formal proofs provided in appendix or supplemental material.
        \item Theorems and Lemmas that the proof relies upon should be properly referenced. 
    \end{itemize}

    \item {\bf Experimental Result Reproducibility}
    \item[] Question: Does the paper fully disclose all the information needed to reproduce the main experimental results of the paper to the extent that it affects the main claims and/or conclusions of the paper (regardless of whether the code and data are provided or not)?
    \item[] Answer: \answerNA{}.% \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: This is a theoretical paper. %\justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item If the paper includes experiments, a No answer to this question will not be perceived well by the reviewers: Making the paper reproducible is important, regardless of whether the code and data are provided or not.
        \item If the contribution is a dataset and/or model, the authors should describe the steps taken to make their results reproducible or verifiable. 
        \item Depending on the contribution, reproducibility can be accomplished in various ways. For example, if the contribution is a novel architecture, describing the architecture fully might suffice, or if the contribution is a specific model and empirical evaluation, it may be necessary to either make it possible for others to replicate the model with the same dataset, or provide access to the model. In general. releasing code and data is often one good way to accomplish this, but reproducibility can also be provided via detailed instructions for how to replicate the results, access to a hosted model (e.g., in the case of a large language model), releasing of a model checkpoint, or other means that are appropriate to the research performed.
        \item While NeurIPS does not require releasing code, the conference does require all submissions to provide some reasonable avenue for reproducibility, which may depend on the nature of the contribution. For example
        \begin{enumerate}
            \item If the contribution is primarily a new algorithm, the paper should make it clear how to reproduce that algorithm.
            \item If the contribution is primarily a new model architecture, the paper should describe the architecture clearly and fully.
            \item If the contribution is a new model (e.g., a large language model), then there should either be a way to access this model for reproducing the results or a way to reproduce the model (e.g., with an open-source dataset or instructions for how to construct the dataset).
            \item We recognize that reproducibility may be tricky in some cases, in which case authors are welcome to describe the particular way they provide for reproducibility. In the case of closed-source models, it may be that access to the model is limited in some way (e.g., to registered users), but it should be possible for other researchers to have some path to reproducing or verifying the results.
        \end{enumerate}
    \end{itemize}


\item {\bf Open access to data and code}
    \item[] Question: Does the paper provide open access to the data and code, with sufficient instructions to faithfully reproduce the main experimental results, as described in supplemental material?
    \item[] Answer: \answerNA{} %\answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: This paper does not include experiments.  %\justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that paper does not include experiments requiring code.
        \item Please see the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item While we encourage the release of code and data, we understand that this might not be possible, so “No” is an acceptable answer. Papers cannot be rejected simply for not including code, unless this is central to the contribution (e.g., for a new open-source benchmark).
        \item The instructions should contain the exact command and environment needed to run to reproduce the results. See the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item The authors should provide instructions on data access and preparation, including how to access the raw data, preprocessed data, intermediate data, and generated data, etc.
        \item The authors should provide scripts to reproduce all experimental results for the new proposed method and baselines. If only a subset of experiments are reproducible, they should state which ones are omitted from the script and why.
        \item At submission time, to preserve anonymity, the authors should release anonymized versions (if applicable).
        \item Providing as much information as possible in supplemental material (appended to the paper) is recommended, but including URLs to data and code is permitted.
    \end{itemize}


\item {\bf Experimental Setting/Details}
    \item[] Question: Does the paper specify all the training and test details (e.g., data splits, hyperparameters, how they were chosen, type of optimizer, etc.) necessary to understand the results?
    \item[] Answer: \answerNA{}. %\answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: This paper does not include experiments. %\justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The experimental setting should be presented in the core of the paper to a level of detail that is necessary to appreciate the results and make sense of them.
        \item The full details can be provided either with the code, in appendix, or as supplemental material.
    \end{itemize}

\item {\bf Experiment Statistical Significance}
    \item[] Question: Does the paper report error bars suitably and correctly defined or other appropriate information about the statistical significance of the experiments?
    \item[] Answer: \answerNA{}. %\answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: This paper does not include experiments. %\justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The authors should answer "Yes" if the results are accompanied by error bars, confidence intervals, or statistical significance tests, at least for the experiments that support the main claims of the paper.
        \item The factors of variability that the error bars are capturing should be clearly stated (for example, train/test split, initialization, random drawing of some parameter, or overall run with given experimental conditions).
        \item The method for calculating the error bars should be explained (closed form formula, call to a library function, bootstrap, etc.)
        \item The assumptions made should be given (e.g., Normally distributed errors).
        \item It should be clear whether the error bar is the standard deviation or the standard error of the mean.
        \item It is OK to report 1-sigma error bars, but one should state it. The authors should preferably report a 2-sigma error bar than state that they have a 96\% CI, if the hypothesis of Normality of errors is not verified.
        \item For asymmetric distributions, the authors should be careful not to show in tables or figures symmetric error bars that would yield results that are out of range (e.g. negative error rates).
        \item If error bars are reported in tables or plots, The authors should explain in the text how they were calculated and reference the corresponding figures or tables in the text.
    \end{itemize}

\item {\bf Experiments Compute Resources}
    \item[] Question: For each experiment, does the paper provide sufficient information on the computer resources (type of compute workers, memory, time of execution) needed to reproduce the experiments?
    \item[] Answer: \answerNA{}. %\answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: This paper does not include experiments. %\justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The paper should indicate the type of compute workers CPU or GPU, internal cluster, or cloud provider, including relevant memory and storage.
        \item The paper should provide the amount of compute required for each of the individual experimental runs as well as estimate the total compute. 
        \item The paper should disclose whether the full research project required more compute than the experiments reported in the paper (e.g., preliminary or failed experiments that didn't make it into the paper). 
    \end{itemize}
    
\item {\bf Code Of Ethics}
    \item[] Question: Does the research conducted in the paper conform, in every respect, with the NeurIPS Code of Ethics \url{https://neurips.cc/public/EthicsGuidelines}?
    \item[] Answer: \answerYes{}.%\answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The research conducted in the paper conforms, in every respect, with the NeurIPS Code of Ethics.
    % This is a theoretical work.  %\justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the authors have not reviewed the NeurIPS Code of Ethics.
        \item If the authors answer No, they should explain the special circumstances that require a deviation from the Code of Ethics.
        \item The authors should make sure to preserve anonymity (e.g., if there is a special consideration due to laws or regulations in their jurisdiction).
    \end{itemize}


\item {\bf Broader Impacts}
    \item[] Question: Does the paper discuss both potential positive societal impacts and negative societal impacts of the work performed?
    \item[] Answer: \answerNA{} %\answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: This is a theoretical work. There is no societal impact of the work performed.%\justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that there is no societal impact of the work performed.
        \item If the authors answer NA or No, they should explain why their work has no societal impact or why the paper does not address societal impact.
        \item Examples of negative societal impacts include potential malicious or unintended uses (e.g., disinformation, generating fake profiles, surveillance), fairness considerations (e.g., deployment of technologies that could make decisions that unfairly impact specific groups), privacy considerations, and security considerations.
        \item The conference expects that many papers will be foundational research and not tied to particular applications, let alone deployments. However, if there is a direct path to any negative applications, the authors should point it out. For example, it is legitimate to point out that an improvement in the quality of generative models could be used to generate deepfakes for disinformation. On the other hand, it is not needed to point out that a generic algorithm for optimizing neural networks could enable people to train models that generate Deepfakes faster.
        \item The authors should consider possible harms that could arise when the technology is being used as intended and functioning correctly, harms that could arise when the technology is being used as intended but gives incorrect results, and harms following from (intentional or unintentional) misuse of the technology.
        \item If there are negative societal impacts, the authors could also discuss possible mitigation strategies (e.g., gated release of models, providing defenses in addition to attacks, mechanisms for monitoring misuse, mechanisms to monitor how a system learns from feedback over time, improving the efficiency and accessibility of ML).
    \end{itemize}
    
\item {\bf Safeguards}
    \item[] Question: Does the paper describe safeguards that have been put in place for responsible release of data or models that have a high risk for misuse (e.g., pretrained language models, image generators, or scraped datasets)?
    \item[] Answer: \answerNA{}. %\answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The paper poses no such risks. % \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper poses no such risks.
        \item Released models that have a high risk for misuse or dual-use should be released with necessary safeguards to allow for controlled use of the model, for example by requiring that users adhere to usage guidelines or restrictions to access the model or implementing safety filters. 
        \item Datasets that have been scraped from the Internet could pose safety risks. The authors should describe how they avoided releasing unsafe images.
        \item We recognize that providing effective safeguards is challenging, and many papers do not require this, but we encourage authors to take this into account and make a best faith effort.
    \end{itemize}

\item {\bf Licenses for existing assets}
    \item[] Question: Are the creators or original owners of assets (e.g., code, data, models), used in the paper, properly credited and are the license and terms of use explicitly mentioned and properly respected?
    \item[] Answer: \answerNA. % \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification:  This paper does not use existing assets. %\justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not use existing assets.
        \item The authors should cite the original paper that produced the code package or dataset.
        \item The authors should state which version of the asset is used and, if possible, include a URL.
        \item The name of the license (e.g., CC-BY 4.0) should be included for each asset.
        \item For scraped data from a particular source (e.g., website), the copyright and terms of service of that source should be provided.
        \item If assets are released, the license, copyright information, and terms of use in the package should be provided. For popular datasets, \url{paperswithcode.com/datasets} has curated licenses for some datasets. Their licensing guide can help determine the license of a dataset.
        \item For existing datasets that are re-packaged, both the original license and the license of the derived asset (if it has changed) should be provided.
        \item If this information is not available online, the authors are encouraged to reach out to the asset's creators.
    \end{itemize}

\item {\bf New Assets}
    \item[] Question: Are new assets introduced in the paper well documented and is the documentation provided alongside the assets?
    \item[] Answer: \answerNA{}. % \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: This paper does not release new assets. %\justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not release new assets.
        \item Researchers should communicate the details of the dataset/code/model as part of their submissions via structured templates. This includes details about training, license, limitations, etc. 
        \item The paper should discuss whether and how consent was obtained from people whose asset is used.
        \item At submission time, remember to anonymize your assets (if applicable). You can either create an anonymized URL or include an anonymized zip file.
    \end{itemize}

\item {\bf Crowdsourcing and Research with Human Subjects}
    \item[] Question: For crowdsourcing experiments and research with human subjects, does the paper include the full text of instructions given to participants and screenshots, if applicable, as well as details about compensation (if any)? 
    \item[] Answer: \answerNA{}. %\answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: This paper does not involve crowdsourcing nor research with human subjects. %\justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Including this information in the supplemental material is fine, but if the main contribution of the paper involves human subjects, then as much detail as possible should be included in the main paper. 
        \item According to the NeurIPS Code of Ethics, workers involved in data collection, curation, or other labor should be paid at least the minimum wage in the country of the data collector. 
    \end{itemize}

\item {\bf Institutional Review Board (IRB) Approvals or Equivalent for Research with Human Subjects}
    \item[] Question: Does the paper describe potential risks incurred by study participants, whether such risks were disclosed to the subjects, and whether Institutional Review Board (IRB) approvals (or an equivalent approval/review based on the requirements of your country or institution) were obtained?
    \item[] Answer: \answerNA{}. %\answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: This paper does not involve crowdsourcing nor research with human subjects. %\justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Depending on the country in which research is conducted, IRB approval (or equivalent) may be required for any human subjects research. If you obtained IRB approval, you should clearly state this in the paper. 
        \item We recognize that the procedures for this may vary significantly between institutions and locations, and we expect authors to adhere to the NeurIPS Code of Ethics and the guidelines for their institution. 
        \item For initial submissions, do not include any information that would break anonymity (if applicable), such as the institution conducting the review.
    \end{itemize}

\end{enumerate}



==> neurips/full-information.tex <==
\section{Adversarial Low-rank MDPs with Full Information}
\label{sec:full-info}
In this section, we discuss adversarial low-rank MDPs with full information. This setting aligns with~\cite{zhao2024learning}, and our \cref{alg:full-info} successfully improve their regret from 
$T^{\nicefrac{5}{6}}$ to  $\sqrt{T}$ with the price of higher computational complexity. We consider model-based learning, with the corresponding assumption formalized in the \cref{assm: model-base} below. This assumption is standard which also appears in prior works on model-based learning in low-rank MDPs ~\citep{agarwal2020flambe, uehara2021representation, zhang2022making, cheng2023improved, zhao2024learning}.
% \begin{assumption}[Model-based Assumption]\label{assm: model-base}
% For any $h \in [H]$, the learner gets access to a model space $\cM_h = \{(\phi_h, \mu_h): \phi_h \in \Phi_h, \mu_h \in \Psi_h\}$ such that for any $h \in [H]$, $\phi^\star_h \in \Phi_h$ and $\mu_h \in \Psi_h$. Moreover, for any $h \in [H]$, any $(x,a,x') \in \cX_h \times \cA \times \cX_{h+1}$, any $\phi_h \in \Phi_h$, and any $\mu_h \in \Psi_h$, we have $\|\phi_h(s,a)\|_2 \le 1$,  $\int \phi_h(x,a)^\top \mu_h(x') dx' = 1$  and for any measurable function $g: \cX \to \mathbb{R}^d$ such that $\|g\|_{\infty} \le 1$, we have $\left\|\int \mu_h(x)g(x) dx\right\|_2 \le \sqrt{d}$ for all $h \in [H]$. Denote $\Phi = \bigcup_{h=1}^H \Phi_h$ and $\Psi = \bigcup_{h=1}^H \Psi_h$.
% \end{assumption}

\begin{assumption}[Model-based assumption]\label{assm: model-base}
The learner has access to two model spaces $\Phi$ and $\Upsilon$ such that $\phi^\star \in \Phi$ and $\mu^\star \in \Upsilon$. Moreover, for any $\phi \in \Phi$, $\mu \in \Upsilon$, and $h\in[2\ldotst H]$, we have $\sup_{(x,a)\in \cX\times \cA}\|\phi_{h-1}(x,a)\|\leq 1$, $\sum_{x' \in \cX} \phi_{h-1}(x,a)^\top \mu_{h}(x') = 1$ and  $\|\sum_{x\in \cX}g(x)\cdot \mu_{h}(x)\|\leq \sqrt{d}$, for all $g:\cX\rightarrow [0,1]$.
\end{assumption}

% Our setting aligns with~\cite{zhao2024learning} who get an oracle efficient algorithm with $T^{\nicefrac{5}{6}}$ regret. Our \cref{alg:full-info} successfully achieves $\sqrt{T}$ regret with the price of more computational complexity that scale with the size of transition space $|\Phi||\Psi|$.


The algorithm of \cite{zhao2024learning} combines the policy optimization framework~\citep{shani2020optimistic} with the exploration bonus design developed by~\cite{uehara2021representation}. 
Instead of constructing exploration bonus through \emph{point-wise} uncertainty quantification (for example, quantifying $\|P_h^\star(\cdot\mid x,a) - \hatp_h^t(\cdot\mid x,a)\|_1$ for all $x,a$) which enables point-wise optimism on every state-action pair, \cite{uehara2021representation}'s exploration bonus only ensures optimism at the initial state. This bonus construction has two limitations when applying to regret minimization in the adversarial setting. First, in order to ensure sufficient exploration, \cite{uehara2021representation}'s algorithm requires sampling the actions using a uniform distribution. While this is fine if we only care about the sample complexity in the reward-free setting, it necessarily leads to sup-optimal regret in the regret minimization setting. Second, without point-wise optimism, there is some technical difficulty in the regret analysis that prevents \cite{zhao2024learning} to perform standard regret decomposition for optimistic policy optimization \citep{shani2020optimistic} (see the discussions in Section~3.2 of \cite{zhao2024learning}). To address the second issue, \cite{zhao2024learning} further introduced the epoching mechanism that stabilizes the policy update. Suffering from these two issues, the algorithm of \cite{zhao2024learning} only achieves a regret of $T^{\nicefrac{5}{6}}$ even in the full-information setting. 


%although they solve a suitale policy to play at every round through policy optimization, it is necessary to additionally mix a uniform policy to encourage exploration over transitions in order to ensure the effectiveness of the bonus. Secondly, when using the near-optimism technique, they need to ensure the local policy update at every state has low regret under the occupancy of estimated transition.  Ideally, the transition estimator should be updated every round based on the newly collected data. However, the local policy update is not able to handle such a frequent changes of transition. Therefore, \cite{zhao2024learning} introduces epoching, which only updates transition estimator after serveral episodes. This approach ensures that the adversarial loss in each epoch can be effectively managed by policy optimization. The trade-off is a reduction in the accuracy of transition estimation and representation learning.

%Unlike in standard linear MDPs that utilize exploration bonus to construct point-wise optimism to cancel uncertainty, these exploration bonus in low-rank MDP only ensures ``near-optimism'', providing optimistic estimation only for the value function specifically at the initial state $x_1$. Such kind of bonus is not well suited to adversarial settings, making the algorithms in \cite{zhao2024learning} have two sources of sub-optimality. Firstly, although they solve a suitale policy to play at every round through policy optimization, it is necessary to additionally mix a uniform policy to encourage exploration over transitions in order to ensure the effectiveness of the bonus. Secondly, when using the near-optimism technique, they need to ensure the local policy update at every state has low regret under the occupancy of estimated transition.  Ideally, the transition estimator should be updated every round based on the newly collected data. However, the local policy update is not able to handle such a frequent changes of transition. Therefore, \cite{zhao2024learning} introduces epoching, which only updates transition estimator after serveral episodes. This approach ensures that the adversarial loss in each epoch can be effectively managed by policy optimization. The trade-off is a reduction in the accuracy of transition estimation and representation learning.

To address these issues, we propose to design the exploration bonus based on point-wise uncertainty quantification. The price we pay is that it is unclear whether our algorithm can be implemented in an oracle-efficient manner. The proposed algorithm is \cref{alg:full-info}. In every episode $t$, we first performs maximum likelihood estimation (MLE) to learn the estimated transition $\hatp^t$ using the previously collected data (\cref{line:MLE}). Then, we construct a transition confidence set $\cP^t$ centered around $\hatp^t$ such that the true model $P^\star$ lies in $\cP^t$ with high probability (\cref{line:confidence}). This confidence set follows the design of \cite{uehara2021pessimistic}.
 Our new bonus  $b^t$ is simply set as the width of the confidence set (\cref{line:bonus}). Since both $\hatp^t$ and $P^\star$ are inside $\cP^t$, the width confidence set captures the maximum uncertainty quantification for the learned model, and thus could serve as a point-wise bonus. %However, in contrast to \cite{zhao2024learning}, the calculation of our bonus lacks computationally efficiency. So far, we do not know how to obtain it without suffering more than $|\Phi||\Upsilon|$ computations.


%In \cref{alg:full-info}, we show that point-wise optimism is actually achieveable in low-rank MDP, which then gets rid all previous drawbacks of the bonus designed for near-optimism. In every episode $t$, we first apply maximum likelihood estimation (MLE) to learn the estimated transition $\hatp^t$ using the currect collected data (\cref{line:MLE}). Then, we construct a transition confidence set $\cP^t$ centered around $\hatp^t$ to ensure the true model $P^\star \in \cP^t$ (\cref{line:confidence}). This confidence set follows the design of \cite{uehara2021pessimistic}.
% Our new bonus  $b^t$ is simply set as the width of the confidence set (\cref{line:bonus}). Since both $\hatp^t$ and $P^\star$ are inside $\cP^t$, the width confidence set captures the maximum uncertainty quantification for the learned model, and thus could serve as a point-wise bonus to cancel such uncertainty. However, in contrast to \cite{zhao2024learning}, the calculation of our bonus lacks computationally efficiency. So far, we do not know how to obtain it without suffering more than $|\Phi||\Upsilon|$ computations.

With the estimated transition kernel $\hatp^t$, uncertainty quantification / bonus $b^t$, and full information loss, we perform policy optimization based on exponential weights (\cref{line: exponential weight every state}). The loss estimator $\Qhat^t$ is the Q-function under the esimated transition $\hatp^t$ and the known loss $\ell^t$. We also enhance our bonus to $\Bhat^t$ defined in \cref{line:dilated} by using the dialated bonus technique \citep{luo2021policy, dai2023refined, liu2023towards}, which introduces an additional factor $(1+\frac{1}{H})$ in the Bellman equation to perform more exploration for deeper layers. The guarantee of \cref{alg:full-info} is summarized in \cref{thm:full-info} below.  

%The following procedure in \cref{alg:full-info} is relatively standard based on policy optimization with exponential weights, where the loss estimator $\Qhat^t$ is simply the Q-function under esimated transition $\hatp^t$ and the known loss $\ell^t$. We also enhance our bonus to $\Bhat^t$ defined in \cref{line:dilated} by using the dialated bonus technique \citep{luo2021policy, dai2023refined, liu2023towards}, which introduces an additional dialated factor $(1+\frac{1}{H})$ in the Bellman Equation of $b^t$ to perform more exploration for deeper layers. The guarantee of \cref{alg:full-info} is summarized in \cref{thm:full-info}.  

\begin{algorithm}[t]
\caption{Model-Based Algorithm for Full-Information Feedback}\label{alg:full-info}
\begin{algorithmic}[1]
    \State Let $\eta = \frac{1}{13H^3\sqrt{T}}$, $\pi^1$ be a uniform policy, $\Bhat^t_{H}(x,a) = b^t_H(x,a) = 0$ for all $x \in \cX, a \in \cA, t \in [T]$. 
    \For{$t=1,2,\ldots, T$}
     \State Execute policy $\pi^t$ and observe trajectory $(\x_{1:H},\a_{1:H})$ and full information loss $\ell^t$.
     \label{line:policy}
     \For{$h=H-1,\dots, 1$}  %\zm{For the edge case $h=H$, we have an issue with $\mu_{H+1}$ and $\x_{H+1}^t$; not defined.} \cwcomment{fixed}
        
        \State Set $\hatp_h^t(x'\mid x,a) = \hphi_h^t(x, a)^\top \hpsi^t_{h+1}(x')$ for all $(x,a,x') \in \cX \times \cA \times \cX$ where \label{line:hatp}
        \begin{align*}
           (\hphi_h^t,\, \hpsi_{h+1}^t) \gets \argmax_{\phi \in \Phi, \mu \in \Upsilon} \sum_{i=1}^t \log \phi(\x_h^i, \a_h^i)^\top \mu(\x_{h+1}^i).
        \end{align*}  \label{line:MLE}
         \State Define confidence set with some large enough universal constant $c$
         \begin{align}
             \cP_h^t = \left\{P \mid  \sum_{i=1}^{t}  \|\hatp_h^t(\cdot\mid \x^i_h, \a^i_h) - P_h(\cdot\mid \x^i_h, \a^i_h)\|_1^2 \le c\log(|\Phi||\Upsilon| T) \right\}. \label{eq:confidence}
         \end{align}  
         \label{line:confidence}
         \State Define $b_h^t(x,a) = 
         2H^2 \max_{P_h, P_h' \in \cP_h^t} \|P_h(\cdot\mid x, a) - P'_h(\cdot\mid x, a)\|_1 
        $ and \label{line:bonus}
         \begin{align}
        \Bhat_h^t(x,a) = b_h^t(x,a) + \left(1+\frac{1}{H}\right) \max_{P_h \in \cP_h^t} \E^{P,\pi^t}\left[\Bhat_{h+1}^t(\x_{h+1},\a_{h+1})\mid \x_h =x,\a_h =a\right]. \label{eq:dilatedbonus}
         \end{align} \label{line:dilated}
     \EndFor
     \State Update policy for all $h\in[H]$: 
     \begin{align*}
             \pi^{t+1}_h(a\mid x) \propto \exp\left( - \eta \sum_{i=1}^{t} \left(\Qhat_h^i(x,a) - \Bhat_h^i(x,a)\right) \right) \ \text{where}\ \Qhat^t_h(x,a) = Q_h^{\hatp^t,\pi^t}(x,a; \ell^t). 
         \end{align*}  \label{line: exponential weight every state}
     
     %\For{$h=1, \ldots, H$}
     %     \State Perform policy evaluation and define $\Qhat^t_h(x,a) = Q_h^{\hatp^t,\pi^t}(x,a; \ell^t)$. \label{line:Qfun}
     %    \State Update policy through exponential weights 
     %    \begin{align*}
      %       \pi^{t+1}_h(a\mid x) \propto \exp\left( - \eta \sum_{i=1}^{t} \left(\Qhat_h^i(x,a) - \Bhat_h^i(x,a)\right) \right). 
      %   \end{align*}  \label{line: exponential weight every state}
      %  \EndFor
    \EndFor
    \end{algorithmic}
\end{algorithm}


\begin{theorem} \label{thm:full-info}
  \cref{alg:full-info} ensures $
     \mathrm{Reg}_T  \le  \otil\left(H^4\sqrt{d|\cA|T} + dH^3|\cA|\right)$.
\end{theorem}

See \cref{app: model based full info} for the proof. In \cite{zhao2024learning}, a lower bound $\Omega\left(H\sqrt{d|\cA|T}\right)$ is derived for this settings when $T \ge d|\cA|$. Thus, our guarantee in  \cref{thm:full-info} matches this lower bound for all $d, |\cA|$ and $T$ up to logarithmic factors.


One technical difference in our analysis compared with \cite{zhao2024learning} is the way to bound the overhead caused by the bonus. The overhead of bonus is typically a generalization error for online data (i.e. $\sum_{t=1}^T\E^{\pi^t}[b_h^t(\x_h,\a_h)]$) while it is usually guaranteed that the bonus $b^t$ has small in-sample error over the data collected till $t-1$ episodes (i.e. $\sum_{i=1}^{t-1}\E^{\pi^i}[b_h^t(\x_h,\a_h)]$ is small). Thus, a change-of-measure happens here and it is usually handled by the elliptical potential lemma, which is also the case in \cite{zhao2024learning}. Recently, \cite{xie2022role} showed that for the MDPs such that the occupancy induced by any policy could be covered by a fixed distribution, the change-of-measure could happen for any function. We show that low-rank MDPs actually have such ``coverability'' property, and small in-sample error guaranteed by MLE directly leads to well-bounded overhead of the bonus.


% Note that in \cite{zhao2024learning}, a lower bound $\Omega(H\sqrt{d|\cA|T})$ is derived for the same setting. Thus, the regret guarantee of \cref{alg:full-info} is for all $d,|\cA|$ and $T$ if $T \ge d|\cA|$.

==> neurips/macro.tex <==
%\usepackage[usenames]{color} %used for font color
\usepackage{makecell}
\usepackage{enumitem}
\newcommand{\cwcomment}[1]{{\color{brown} [cw:#1]}}
\usepackage[usenames]{color} %used for font color
\usepackage{amssymb} %maths
\usepackage{mathtools}
\usepackage{amsthm}
\usepackage{amsmath} %maths
\allowdisplaybreaks
\usepackage[utf8]{inputenc} 
\usepackage{bm}
\usepackage{bbm}
%\usepackage[ruled, linesnumbered, vlined]{algorithm2e}
\usepackage{algorithm}
\usepackage{algpseudocode}
\usepackage{algorithmicx}
\usepackage{MnSymbol}
\usepackage{comment}
\usepackage{setspace}
\usepackage{url}            % simple URL typesetting
\usepackage{booktabs}       % professional-quality tables
%\usepackage{amsfonts}       % blackboard math symbols
\usepackage{nicefrac}       % compact symbols for 1/2, etc.
\usepackage{microtype}      % microtypography
\usepackage{parskip}


\input{../widebar.tex}


%%%%%%%%%%%% cleverref %%%%%%%%% 
\usepackage{hyperref}
\usepackage[nameinlink,capitalize]{cleveref}
\usepackage{crossreftools}
\makeatletter
\newcommand{\neutralize}[1]{\expandafter\let\csname c@#1\endcsname\count@}
\makeatother

   \newenvironment{lemmod}[2]
  {\renewcommand{\thelemma}{\ref*{#1}#2}%
   \neutralize{lemma}\phantomsection
   \begin{lemma}}
  {\end{lemma}}


\newenvironment{thmmod}[2]
  {\renewcommand{\thetheorem}{\ref*{#1}#2}%
   \neutralize{theorem}\phantomsection
   \begin{theorem}}
  {\end{theorem}}


\newenvironment{bodythmmod}[2]
  {\renewcommand{\thebodytheorem}{\ref*{#1}#2}%
   \neutralize{bodytheorem}\phantomsection
   \begin{theorem}}
  {\end{theorem}}

    \newenvironment{propmod}[2]
  {\renewcommand{\theproposition}{\ref*{#1}#2}%
   \neutralize{proposition}\phantomsection
   \begin{proposition}}
  {\end{proposition}}

     \newenvironment{defnmod}[2]
  {\renewcommand{\thedefinition}{\ref*{#1}#2}%
   \neutralize{definition}\phantomsection
   \begin{definition}}
  {\end{definition}}

   \newenvironment{asmmod}[2]
  {\renewcommand{\theassumption}{\ref*{#1}#2}%
   \neutralize{assumption}\phantomsection
   \begin{assumption}}
  {\end{assumption}}

  \newenvironment{cormod}[2]
  {\renewcommand{\thecorollary}{\ref*{#1}#2}%
   \neutralize{corollary}\phantomsection
   \begin{corollary}}
  {\end{corollary}}
  
   \newenvironment{condmod}[2]
  {\renewcommand{\thecondition}{\ref*{#1}#2}%
   \neutralize{condition}\phantomsection
   \begin{condition}}
  {\end{condition}}

\pdfstringdefDisableCommands{%
    \let\Cref\crtCref
    \let\cref\crtcref
}
\newcommand{\creftitle}[1]{\crtcref{#1}}

\makeatletter
\renewenvironment{proof}[1][Proof]%
{%
	\par\noindent{\bfseries\upshape {#1.}\ }%
}%
{\qed\newline}
\makeatother
\creflabelformat{line}{#2\textup{#1}#3} 

%%%%%%%%%% End of ref %%%%%%%
\usepackage{thmtools}
\declaretheorem[name=Theorem, numberwithin=section]{thm}
\declaretheorem[name=Theorem,parent=section]{theorem}
\declaretheorem[name=Lemma,parent=section]{lemma}
\declaretheorem[name=Definition,parent=section]{definition}
\declaretheorem[name=Corollary,parent=section]{corollary}
\declaretheorem[name=Claim,parent=section]{claim}
\declaretheorem[name=Assumption, parent=section]{assumption}
\declaretheorem[name=Condition, parent=section]{condition}
%\declaretheorem[qed=$\triangleleft$,name=Example,style=definition, parent=section]{example}
\declaretheorem[name=Remark,parent=section]{remark}
\declaretheorem[name=Proposition, parent=section]{proposition}
\declaretheorem[name=Fact, parent=section]{fact}

\usepackage{transparent}
\usepackage{xcolor}
\newcommand{\algcomment}[1]{\textcolor{blue!70!black}{\small{\texttt{\textbf{//\hspace{2pt}#1}}}}}
\newcommand{\algcommentlight}[1]{\textcolor{blue!70!black}{\transparent{0.5}\footnotesize{\texttt{\textbf{//\hspace{2pt}#1}}}}}
\newcommand{\algcommentbig}[1]{\textcolor{blue!70!black}{\footnotesize{\texttt{\textbf{/*
					#1~*/}}}}}
\newcommand{\algcommentbiglight}[1]{\textcolor{blue!70!black}{\transparent{0.5}\footnotesize{\texttt{\textbf{/* #1~*/}}}}}
\newcommand{\algcolor}[1]{\textcolor{blue!70!black}{#1}}
\newcommand{\algspace}{\hspace{\algorithmicindent}}
%\newcommand{\algcomment}[1]{\Statex \textcolor{blue}{// #1 //}}
\newcommand{\Input}{\item[\textbf{Input:}]}

\usepackage{color-edits}
\addauthor{zm}{red}
\newcommand{\zm}[1]{\textcolor{red}{#1}}
\newcommand{\jz}[1]{\textcolor{blue}{JZ:#1}}

%%%%%%%%%% End of ref %%%%%%%


\newcommand{\cP}{\mathcal{P}}
\newcommand{\E}{\mathbb{E}}
\renewcommand{\P}{\mathbb{P}}
\newcommand{\cA}{\mathcal{A}}
\newcommand{\veps}{\varepsilon}
\newcommand{\pistar}{\pi^\star}
\newcommand{\reg}{\mathrm{reg}}
\newcommand{\Bhat}{\widehat{B}}
\newcommand{\bell}{\bm{\ell}}
\newcommand{\replearn}{\texttt{replearn}}
\newcommand{\rep}{\mathrm{rep}}
\newcommand{\pibar}{\bar{\pi}}
\newcommand{\Qbar}{\widebar{Q}}
\newcommand{\what}{\widehat{w}}
\newcommand{\pihat}{\widehat{\pi}}
\newcommand{\x}{\bm{x}}
\renewcommand{\a}{\bm{a}}
\newcommand{\phistar}{\phi^\star}
\newcommand{\dd}{\mathrm{d}}
\newcommand{\rl}{\mathrm{repl}}
\newcommand{\phirl}{\phihat^{\rl}}
\newcommand{\Qhat}{\widehat{Q}}
\newcommand{\ind}[1]{^{(#1)}}

\newcommand{\mustar}{\mu^\star}
\newcommand{\nn}{\nonumber}
\newcommand{\phihat}{\hat{\phi}}
\newcommand{\cX}{\mathcal{X}}
\newcommand{\cG}{\mathcal{G}}
\newcommand{\cB}{\mathcal{B}}
\newcommand{\reals}{\mathbb{R}}
\newcommand{\nreg}{N_\mathrm{reg}}
\newcommand{\cD}{\mathcal{D}}
\newcommand{\Sigmahat}{\widehat{\Sigma}}
\newcommand{\order}{\mathcal{O}}
\newcommand{\hphi}{\hat{\phi}}
\newcommand{\hpsi}{\hat{\mu}}
\newcommand{\hd}{\hat{d}}
\newcommand{\hV}{\widehat{V}}
\newcommand{\hell}{\hat{\ell}}
\newcommand{\tr}{\text{\rm Tr}}
\newcommand{\td}{\Tilde{d}}
\newcommand{\indi}{\mathbbm{1}}
\newcommand{\cZ}{\mathcal{Z}}
\newcommand{\cM}{\mathcal{M}}
\newcommand{\otil}{\widetilde{\mathcal{O}}}
\newcommand{\Vhat}{\widehat{V}}

\DeclareMathOperator*{\argmin}{argmin}
\DeclareMathOperator*{\argmax}{argmax}
\newcommand{\unif}{\texttt{unif}}
\newcommand{\ldotst}{%
	\mathinner{{\ldotp}{\ldotp}}%
}
\newcommand{\wtilde}{\widetilde}
%\newcommand{\phibar}{\bar{\phi}}
\newcommand{\cF}{\mathcal{F}}
\newcommand{\cC}{\mathcal{C}}
\newcommand{\cQ}{\mathcal{Q}}
\newcommand{\cH}{\mathcal{H}}
\newcommand{\fhat}{\hat{f}}
\newcommand{\vepsstatval}{c \cdot \frac{d\log(N_\reg K H/\delta)}{N_\reg}}
\newcommand{\vepsregval}{\frac{5H^3d^2\log(2 K H^2 d |\Phi| /\delta)}{N_\reg}}
\newcommand{\vepsregvalB}{\frac{37H^2d^2\beta^2\log(6 K H^2 d|\Phi| \delta^{-1} \gamma^{-1})}{N_\reg}}
\newcommand{\stat}{\mathrm{stat}}
\newcommand{\cov}{\mathrm{cov}}
\newcommand{\indd}[1]{^{#1}}
\newcommand{\cL}{\mathcal{L}}
\newcommand{\cI}{\mathcal{I}}
\newcommand{\bpi}{\bm{\pi}}
\newcommand{\cU}{\mathcal{U}}
\renewcommand{\u}{\bm{u}}
\newcommand{\z}{\bm{z}}
\newcommand{\bcH}{\bm{\cH}}
\newcommand{\thetahat}{\hat\theta}
\newcommand{\spanner}{\mathrm{span}}
\newcommand{\bzeta}{\bm{\zeta}}
\newcommand{\bh}{\bm{h}}
\newcommand{\est}{\texttt{LinEst}}
\newcommand{\psdp}{\texttt{PSDP}}
\newcommand{\estmat}{\texttt{EstMat}}
\newcommand{\veceval}{\texttt{EstVec}}
\newcommand{\rspanner}{\texttt{RobustSpanner}}
\newcommand{\apx}{\texttt{LinOpt}}
\newcommand{\btheta}{\bm{\theta}}
\newcommand{\bvartheta}{\tilde{\btheta}}
\newcommand{\Trepval}{\frac{A H \log(|\Phi|/\delta)}{\alpha \veps^2}}
\newcommand{\Tspanval}{\frac{A \log(d H|\Phi|\veps^{-1} \delta^{-1} )}{\alpha \veps^2}}
\newcommand{\Trepvalf}{\alpha^{-1}\veps^{-2} A H \log(|\Phi|/\delta)}
\newcommand{\Tspanvalf}{\alpha^{-2} \veps^{-2} A \log(d H|\Phi|\veps^{-1} \delta^{-1} )}
\newcommand{\Tcovval}{\veps^{-2}A d^{13} H^6 \log(\Phi/\delta)}
\newcommand{\loss}{\mathrm{loss}}
\newcommand{\freed}{\mathrm{freed}}
\newcommand{\phib}{\bar{\phi}}
\newcommand{\phibar}{\bar{\phi}}
\newcommand{\thetab}{\bar{\theta}}
\newcommand{\ww}{w}
\newcommand{\g}{g}
\newcommand{\varthetab}{\bm{\vartheta}}
\newcommand{\bvthetab}{\bar{\varthetab}}
\newcommand{\thetabar}{\bar{\theta}}

\newcommand{\tB}{\wtilde{B}}

\newcommand{\tb}{\wtilde{b}}

\newcommand{\tp}{\wtilde{P}}

\newcommand{\hatell}{\hat{\ell}}
\newcommand{\hatphi}{\hat{\phi}}
\newcommand{\hatmu}{\hat{\mu}}
\newcommand{\tilp}{\rho}
\newcommand{\hatp}{\widehat{P}}
\newcommand{\var}{\text{\rm Var}}
\newcommand{\bbB}{\mathbb{B}}
\newcommand{\calZ}{\mathcal{Z}}
\newcommand{\poly}{\mathrm{poly}}
\newcommand{\cE}{\mathcal{E}}
\newcommand{\john}{\texttt{John}}





==> neurips/model-based-bandit.tex <==
\section{Inefficient Model-Based Algorithm with Bandit Feedback} \label{sec:model-based bandit}
In this section, we go beyond the full-information setting and derive the first (model-based) algorithm (\cref{alg:low-rank bandit}) for adversarial low-rank MDPs with sublinear regret. Compared with linear MDPs, the key challenge for more general low-rank MDPs is to construct a proper loss estimator. For linear MDP, since the feature is known, the loss estimator closely resembles that of linear bandits. However, low-rank MDPs lack such structural simplicity, making standard loss estimators invalid. To overcome this challenge, we propose a new loss estimator that works for any loss function based on off-policy evaluation and the low-rank structure of transition. In this section, $\otil$ hides logarithmic factors of $d,H,T, |\Phi||\Upsilon|$.


In \cref{alg:low-rank bandit}, we first conduct an initial representation learning phase to establish accurate transition estimator $\hatp$  and its corresponding features $\hphi$ and $\hpsi$ based on reward-free exploration algorithms in \cite{cheng2023improved}. Different from the reward-free setting, our downstream task is to handle adversarial losses. Thus, we use exponential weights to maintain a distribution over the policy space $\Pi'$ where we mix a uniform policy with  $\Pi$ to enhance exploration. At every round $t$, a behavior policy $\pi^t$ is chosen from the current policy distribution, and we use the data collected by $\pi^t$ to estimate the value for every $\pi \in \Pi'$. The success of such off-policy evaluation is based on the following observations of low-rank MDP. Using the low-rank transition structure, for $h \ge 2$, we have 
\begin{align} \label{eqn:low-rank}
  \forall \pi\in \Pi,\quad   d_h^{\pi}(x) =  \phi_{h-1}^\star(\pi)^\top \mu_{h}^\star(x),\quad \text{where}\quad \phi_{h-1}^\star(\pi) \coloneqq \E^{\pi}[\phistar_{h-1}(\x_{h-1},\a_{h-1})].
\end{align}
Thus, using the definition of the $V$-function from \cref{sec:prelim}, we have for any loss function $\ell$ and $\pi$:
\begin{align} \label{eqn:V dec}
    V^{\pi}_1(x_1; \ell)- \E[\ell_1(\x_1,\a_1)]= \sum_{h=2}^H \sum_{(x,a)\in \cX\times \cA}  \phi_{h-1}^{\star} (\pi)^\top \mu_{h}^\star(x) \pi_h(a\mid x)\cdot \ell_h(x,a).
\end{align}
Letting $\Lambda_h^t \coloneqq (\E_{\bpi^t \sim p^t}\left[\phi_h^\star(\bpi^t)\phi_h^{\star}(\bpi^t)^\top\right])^{-1}$ and ingnoring the loss term $\E[\ell_1(\x_1,\a_1)]$ from the first step (this term can easily be treated as in a bandit setting with $H=1$), we have for all $\pi\in \Pi'$:
\begin{align*}
     V_1^{\pi}(x_1; \ell)  &=  \E_{\bpi^t \sim p^t}\left[\sum_{h=2}^H \sum_{(x,a)\in \cX\times \cA}  \phi_{h-1}^{\star} (\pi)^\top\Lambda_{h-1}^t \phi_{h-1}^\star(\bpi^t)\phi_{h-1}^{\star}(\bpi^t)^\top \mu_{h}^\star(x) \pi_h(a\mid x)\cdot \ell_h(x,a)\right],
    \\&= \E_{\bpi^t \sim p^t}\left[\sum_{h=2}^H \sum_{x,a}  \phi_{h-1}^{\star} (\pi)^\top \Lambda_{h-1}^t \phi_{h-1}^\star(\bpi^t)\cdot d_h^{\bpi^t}(x)\bpi_h^t(a\mid x)\frac{\pi_h(a\mid x)}{\bpi_h^t(a\mid x)}\cdot \ell_h(x,a)\right],
    \\&= \E_{\bpi^t \sim p^t}\E^{\bpi^t}\left[ \sum_{h=2}^H \phi_{h-1}^{\star}(\pi)^\top\Lambda_{h-1}^t \phi_{h-1}^\star(\bpi^t)\cdot \frac{\pi_h(\a_h\mid \x_h)}{\bpi_h^t(\a_h\mid \x_h)}\cdot \ell_h(\x_h,\a_h)\right].
\end{align*}
Thus, for all $\ell$ and $\pi$, $\sum_{h=2}^H \phi_{h-1}^{\star}(\pi)^\top\Lambda_{h-1}^t \phi_{h-1}^\star(\bpi^t)\cdot {\pi_h(\a_h\mid \x_h)}\bpi_h^t(\a_h\mid \x_h)^{-1}\cdot \ell_h(\x_h,\a_h)$ for $\bpi^t\sim p^t$ and $(\x_h,\a_h)\sim d^{\bpi^t}_h$ is an unbiased estimator of $V^\pi_1(x_1, \ell)$. However, $\phi_{h-1}^\star(\pi)$ is not accessible because both the true feature $\phi^\star$ and occupancy $d^\pi$ for the true transition are unknown. Thus, our estimator incorporates the learned feature $\hphi$ and the occupancy of $\hatp$ instead as shown in \cref{line:est feature} and \cref{line:bandit estimator}. Utilizing estimated features and transition could introduce additional bias but the initial representation learning already ensures such bias is small enough to tackle. We compensate for the bias by incorporating a well-designed exploration bonus $b^t(\pi)$ in exponential weights when conducting policy distribution updates. To further encourage exploration, we additionally perform John's exploration together with exponential weights when selecting behavior policies. The main guarantee of \cref{alg:low-rank bandit} is given in \cref{thm:model-based bound}.



% This technique is also widely used in learning adversarial linear MDPs ~\citep{luo2021policy, dai2023refined, saha2020improved, kong2023improved, liu2023towards}. 



% and technically speaking, introduce boundness property to our loss estimator, we additionally mix a uniform distribution in our policy space and perform John's exploration together with exponential weights when selecting behaviour policies. 



% Let $\Pi$ be policy set in which every policy is a mixture of a deterministic policy and $\beta$ uniform distribution.

\begin{algorithm}
\caption{Model-Based Algorithm for Bandit Feedback} \label{alg:low-rank bandit}
\begin{algorithmic}[1]
    \Input A policy class $\Pi$. 
    \State Set $\epsilon = T^{-\frac{1}{3}}$, $\gamma = T^{-\frac{1}{3}}$, $\beta = T^{-\frac{1}{3}}$, $\eta = ({4Hd|\cA|})^{-1} T^{-\frac{2}{3}}$, and $T_0 = \otil( \epsilon^{-2}H^3d^2|\cA|(d^2 + |\cA|))$.
    \State Run \cite[Algorithm 1]{cheng2023improved} for $T_0$ episodes and get outputs $\hphi \in \Phi, \hpsi \in \Upsilon$. 
    \State Define transitions $\hatp_{1:H-1}$ as 
    $$\hatp_h(x'\mid  x,a) = \hphi_h(x,a)^\top \hpsi_{h+1}(x'), \quad \forall (x,a,x') \in \cX \times \cA \times \cX.$$
    \State For all $h\in[H-1]$, define $\hphi_h(\pi) = \sum_{(x,a)\in \cX\times \cA} \hd_{h}^\pi(x,a)\cdot \hphi_{h}(x,a)$, where $\hd_h^\pi \coloneqq d_h^{\hatp,\pi}$. \label{line:est feature}
    \State Define the policy space $\Pi' = \{\pi':~ \exists \pi\in\Pi, \ \ \pi_h'(\cdot\mid x)= (1-\beta)\pi_h(\cdot\mid x) +  \beta/|\cA|, \ \  \forall x, h\}$. %\zm{Define $\pi_\unif$ in prelim} 
    \label{line:mix pi}
    \For{$t = T_0 + 1,\, T_0 + 2,\ldots, T$}
         \State Define $ p^t(\pi) \propto \exp\left(-\eta \sum_{i=1}^{t-1}  \left(\hatell^i(\pi) - b^i(\pi)\right)\right),$ for all $\pi \in \Pi'$. \label{line:bandit-exp}
         \State Let $\tilp^t(\pi) = (1-\gamma)p^t(\pi) +  \frac{\gamma}{H-1}\sum_{h=1}^{H-1}  J_h$, where $J_h = \john(\hatphi_h(\cdot), \Pi')$. \algcommentlight{$\john$ as in \S\ref{sec:prelim}}  %\zm{Do we define \text{John} somewhere? Also use macro john}  \cwcomment{I made some edit here. John's exp defined in prelim}
         \State Execute policy $\bpi^t\sim \tilp^t$ and observe trajectory $(\x^t_{1:H}, \a^t_{1:H})$ and losses $\bell^t_h =\ell^t_h(\x_h^t,\a_h^t)$.
         \State Define $\Sigma^t_{h} = \sum_{\pi \in \Pi'}\tilp^t(\pi)\cdot \hatphi_h(\pi)\hatphi_h(\pi)^\top$, $b^t(\pi) = \sqrt{d}H\epsilon \cdot \sum_{h=1}^{H-1} \|\hatphi_h(\pi)\|_{(\Sigma^t_{h})^{-1}}$, and
             \begin{align*}  
            \hell^t(\pi) = \frac{\pi_1(a_1^t\mid x_1^t)}{\pi_1^t(a_1^t\mid x_1^t)}\bell_1^t + \sum_{h=2}^H \hphi_{h-1}(\pi)^\top\left(\Sigma_{h-1}^t\right)^{-1} \hphi_{h-1}(\pi^t) \frac{\pi_h(a_h^t\mid x_h^t)}{\pi_h^t(a_h^t\mid x_h^t)}\bell_h^t.
             \end{align*} \label{line:bandit estimator}
         \EndFor
    \end{algorithmic}
\end{algorithm}

\begin{theorem}\label{thm:model-based bound}
\cref{alg:low-rank bandit} achieves $\mathrm{Reg}_T(\pi) \le  \otil\left(d^2 H^3 |\cA|(d^2 + |\cA|)T^{\nicefrac{2}{3}}\log|\Pi|\right)$ for any $\pi \in \Pi$.
\end{theorem}

Note that the guarantee in \cref{thm:model-based bound} only holds for policy $\pi \in \Pi$. To ensure our regret bound is meaningful, at least a near-optimal policy should be contained in the given policy set $\Pi$. In general, the size of such a policy set would grow exponentially with the number of states (e.g.~covering of all Markovian policies), which makes the regret has polynomial dependence on the number of states. In \cref{thm:lowerboundmain}, we show that even for low-rank MDPs, if the loss function lacks structure, the regret cannot avoid polynomial dependence on the number of states. The detailed construction for this lower-bound is given in \cref{sec:lower bound}.

\begin{theorem}\label{thm:lowerboundmain}
There exists a low-rank MDP with $|\cX|$ states, $|\cA|$ actions and sufficiently large $T$ with unstructured losses such that any agent suffers at least regret of $\Omega(\sqrt{|\cX| |\cA| T})$.
\end{theorem}


\cref{thm:lowerboundmain} shows that in general, we could not gain too much from low-rank transition structure compared with tabular MDPs. To get rid of any dependence on the number of states, we additonly introduce \cref{assm:linearlossweak} to impose linear structure on the loss function. Unlike standard linear MDPs that require the loss feature is known, our algorithm can even handle linear loss with unknown feature, since we never explicitly use the loss feature and we only need the linear structure to reduce the size of the candidate policy class. Specifically, when both loss and transition are linear, the Q-function is also linear, making it sufficient to consider the following linear policy space
\begin{align*}
    \Pi_{\text{\rm lin}} = \left\{\pi :\cX\rightarrow \cA \ \Big\mid \   \pi_h(a\mid x ) = \mathbb{I}\big\{a=\argmin_{a \in \cA} \phi_h(x, a)^\top \theta_h\big\}, \ h\in[H],\  \|\theta_h\|_2 \le \sqrt{d}H T, \ \phi \in \Phi\right\}.
\end{align*}
The $\frac{1}{T}$-cover of $ \Pi_{\text{\rm lin}}$ only have size $|\Phi|\cdot T^{\mathcal{O}(d)} $ following standard arguments (e.g, Exercise 27.6 of \cite{lattimore2020bandit}) and if we feed it into \cref{alg:low-rank bandit}, our regret could avoid dependece on the size of state space as shown in \cref{cor:linear policy reg}.

\begin{corollary}\label{cor:linear policy reg}
If the loss function satisfies \cref{assm:linearlossweak}, applying \cref{alg:low-rank bandit} with $\Pi$ as the $\frac{1}{T}$-cover of $ \Pi_{\text{\rm lin}}$ ensures $\mathrm{Reg}_T   \le  \otil\left(d^3 H^3 |\cA|(d^2 + |\cA|)T^{\nicefrac{2}{3}}\right)$.
\end{corollary}

==> neurips/model-free.tex <==
In this section, we consider the model-free setting, where we only assume access to a feature class $\Phi$ that contains the true feature map $\phistar$. 
\begin{assumption}[Model-free Realizability]
\label{assm:real}
    The learner has access to a function class $\Phi$ such that
\begin{align}
    \phistar \in \Phi \qquad \text{and} \qquad \sup_{\phi\in \Phi} \sup_{(x,a)\in \cX\times \cA} \|\phi(x,a)\| \leq 1. \label{eq:phibound}
\end{align}
\end{assumption}
This is a standard assumption in the context of model-free RL~\citep{modi2024model, zhang2022efficient, mhammedi2024efficient}. We note that having access to the function class $\Phi$ alone (instead of both $\Phi$ and $\Upsilon$ as in \cref{assm: model-base}) is not sufficient to model the transition probabilities (unlike in the model-based case). This makes the model-free setting much more challenging; in fact, until the recent work by \cite{mhammedi2023efficient} there were no model-free, oracle-efficient algorithms for this setting that do not require any additional structural assumptions on the MDP. 

\subsection{Algorithm Description}
\input{../algorithm_oracle_eff}
We now descibe the key component of our efficient model-free algorithm (\cref{alg:oraceleff}).
\paragraph{Exploration phase and policy cover.}
Similar to algorithms in the previous section, \cref{alg:oraceleff} begins with a reward-free exploratorion phase; \cref{line:explore} of \cref{alg:oraceleff}. However, unlike in the previous sections where the role of this exploration phase was to learn a model for the transition probabilities, here the goal is to compute a, so called, \emph{policy cover} which is a small set of policies that can be used to effectively explore the state space. 
\begin{definition}[Approximate policy cover] 
    \label{def:cover}For $\alpha,\veps\in(0,1]$ and $h\in[H]$, a subset $\Psi\subseteq \Pi$ is an $(\alpha, \veps)$-policy cover for layer $h$ if 
\begin{align}
    \max_{\pi\in \Psi} d_h^{\pi}(x)\geq \alpha \cdot \max_{\pi'\in \Pi} d_h^{\pi'}(x), \quad  \text{for all $x\in \cX$ such that } \max_{\pi'\in \Pi} d^{\pi'}_h(x)\geq \veps \cdot \|\mu^\star_h(x)\|.
\end{align}
\end{definition}
In \cref{line:explore}, \cref{alg:oraceleff} calls $\texttt{VoX}$ \citep{mhammedi2023efficient}, a reward-free and model-free exploration algorithm to compute $(1/(8Ad),\veps)$-policy covers $\Psi_{1}^\cov, \dots ,\Psi_H^\cov$ for layers $1,\dots, H$, respectively, with $|\Psi_h|=d$ for all $h\in[H]$. This call to $\texttt{VoX}$ requires $O(1/\veps^2)$ episodes; see the guarantee of \texttt{VoX}{} in \cref{lem:vox}. 
After this initial phase, the algorithm operates in epochs, each consisting of $N_\reg\in\mathbb{N}$ episodes, where in each epoch $k\in[K]$, the algorithm commits to executing policies sampled from a fixed policy distribution $\rho\ind{k}\in \Delta(\Pi)$ with support on the policy covers $\Psi^\cov_{1:H}$ and a policy $\pihat\ind{k}$ specified by an online learning algorithm. Next, we describe in more detail how $\rho\ind{k}$ is constructed and motivate the elements of its construction starting with the online learning policies $\{\pihat\ind{k}\}_{k\in[K]}$.

\paragraph{Online learning policies.}
Given estimates $\{\Qhat_{1:H}\ind{s}\}_{s<k}$ of the average $Q$-functions \begin{align}\left\{\frac{1}{N_\reg} \sum_{t\text{ in epoch }s} Q^{\pihat\ind{s}}_{1:H}(\cdot,\cdot;\ell^t)\right\}_{s<k}\label{eq:avgQ} \end{align} from the previous epoch (we will descibe how these estimates are computed in the sequel), \cref{alg:oraceleff} computes policy $\pihat\ind{k}$ for epoch $k$ according to 
\begin{align}
 \pihat_h\ind{k}(\cdot)\in \argmin_{\pi \in \Delta(\cA)}\sum_{s < k} \sum_{a\in \cA}  \left(\eta\cdot \pi(a\mid \cdot)\cdot \Qhat\ind{s}_h(\cdot,a) +\log\frac{1}{\pi(a\mid \cdot)}\right), \label{eq:onlinepolicy}
\end{align}
for all $h\in[H]$. Given a state $x\in \cX$, the distribution over actions $\pihat\ind{k}_h(\cdot \mid x)$ represents the output of a certain online learning algorithm that ensures a sublinear regret with respect to the squence of loss functions given by $\{\pi \mapsto \sum_{h\in[H]}\Qhat_{h}\ind{k}(\cdot, \pi_h(\cdot))\}_{k\in[K]}$. Thanks to the performance difference lemma, and as shown in \cite{luo2021policy}, a sublinear regret with respect to these "surrogate" loss functions translates into a sublinear regret in the low-rank MDP game we are interested in, granted that $\{\Qhat_{1:H}\ind{k}\}_{k\in[K]}$ are good estimates of the average $Q$-functions \cite{luo2021policy}. In line with previous analyses, we require the $Q$-function estimates to ensure that the following bias term 
\begin{align}
\E^{\pi}\left[\max_{a\in\cA} \left(\frac{1}{N_\reg}\sum_{t\text{ in epoch } k}Q_h^{\pihat\ind{k}}(\x_h,a;\ell^t)-\Qhat\ind{k}_h(\x_h,a)\right)^2\right] \label{eq:biases}
\end{align}
is small for all $h\in[H]$, $k\in[K]$, and $\pi\in \Pi$. 

\paragraph{$Q$-function estimates.} Thanks to the low-rank MDP structure and the linear loss representation assumption (\cref{assm:linearlossweak}), the avegare $Q$-functions in \eqref{eq:avgQ} are linear in the feature maps $\phistar$. Thus, using the function class $\Phi$ in \cref{assm:normalizing} we can estimate these average $Q$-functions by regressing the sum of losses $\sum_{s=h}^H\bell_s^t$ onto $(\x_h^t,\a_h^t)$ for $t$ in the $k$th epoch (as in \eqref{eq:regproblem0}). However, na\"ively doing this using only trajectories generated by $\pihat\ind{k}$ would only ensure that the bias term in \eqref{eq:biases} is small for $\pi = \pihat\ind{k}$. To ensure that it is small for all possible policies $\pi$'s, we need to estimate the $Q$-functions on the trajectories of policies that are guaranteed to have good state coverage; this is where we use the policy cover from the initial phase. 

\paragraph{Mixture of policies.}
At episode $t$ in each epoch $k\in[K]$, we execute policy $\bpi\ind{k}$ sampled from $\rho\ind{k}$, where $\rho\ind{k}$ is set to be the distribution of the random policy: 
\begin{align}
 \mathbb{I}\{\bzeta\indd{t} = 0\} \cdot  \pihat\ind{k}+ \mathbb{I}\{\bzeta\indd{t} = 1\} \cdot \bpi\indd{t}\circ_{\bh\indd{t}}   \pi_\unif \circ_{\bh\indd{t}+1} \pihat\ind{k}, \label{eq:this}
 \end{align}
with $\bzeta\indd{t} \sim \mathrm{Ber}(\nu)$, $\bh\indd{t}\sim \unif([H])$, and $\bpi\indd{t} \sim \unif(\Psi^{\texttt{cov}}_{\bh\indd{t}})$. In words, at the start of each episode of any epoch $k$, we execute $\pihat\ind{k}$ (see \eqref{eq:onlinepolicy}) with probability $1-\nu$; and with probability $\nu$, we execute a policy in $\Psi^\cov_{1:H}$ selected uniformly at random. As explained in the previous paragraph, this ensures a small bias for all choices of $\pi$ in \eqref{eq:biases} thanks the policy cover property of $\Psi^\cov_{1:H}$. 

\subsection{Algorithm Guarantee}
We now state the guarantee of \cref{alg:oraceleff}. 
\begin{theorem}
\label{thm:oraclealg}
Let $\delta\in(0,1)$ be given. For $T = \mathrm{poly}(A,d,H, \log(|\Phi|/\delta))$ sufficiently large, \cref{alg:oraceleff} guarantees $\mathrm{Reg}_T \leq \poly(A,d,H,\log(|\Phi|/\delta))\cdot T^{\nicefrac{5}{6}}$ regret against an oblivious adversary.
\end{theorem}
The proof is in \cref{sec:oracleeff}. Note that the $T$-dependence in this regret matches that of the previous best bound by \cite{zhao2024learning} (see \cref{tab:comparison}). Compared to their algorithm, \cref{alg:oraceleff} is model-free and only requires bandit feedback. This makes the result in \cref{thm:oraclealg} rather surprising.


\subsection{Extention to Adaptive Adversary}
\label{sec:extension}
%\zm{In progress} This algorithm also starts with an exploration phase, where it calls \texttt{VoX} \cite{mhammedi2023efficient} to learn a policy cover; \texttt{VoX} is a model-free, reward-free exploration algorithm. After this initial exploratory phase, the algorithm operates in epochs; during epoch $k$, the algorithm commits to a fixed mixture of policies. This mixture consists of certain exploratory policies (based on the policy cover from the initial phase) and a policy computed using an online learning algorithm based on estimated $Q$-functions from previous epochs (these act as loss functions). Mixing with eploratory policies is needed here to estimate the $Q$-functions that the online algorithm uses. 
 In \cref{sec:adaptive}, we modify \cref{alg:oraceleff} algorithm to handle the much more challenging setting of an \emph{adaptive} adversary with bandit feedback. Here, we make the additional assumption that the losses are linear with respect to a \emph{known} feature $\phi^\loss$, which may be different from the feature of the low-rank decomposition (see \cref{assm:linearloss}). The new algorithm (\cref{alg:algorithm_name} deferred to the appendix due to space) is similar to \cref{alg:oraceleff} with the following key differences; after computing a policy cover, the algorithm calls $\texttt{RepLearn}$ to compute a feature map $\phi^\rep$. Then, for every $h\in[H]$, the algorithm computes a \emph{spanner}; a set of policies $\Psi^\spanner_h =\{\pi_{h,1},\dots,\pi_{h,2d}\}$ that act as an approximate spanner for the set $\{\E^{\pi}[\phi^\rep_h(\x_h,\a_h), \phi^\loss_h(\x_h,\a_h)]:\pi \in \Pi\}\subseteq \reals^{2d}$, where we use $[\cdot,\cdot]$ to denote the vertical concatenation of vectors. These spanner policies are then used as the exploratory policies after the initial phase; that is, we use $\bpi^t\sim \unif(\Psi^\spanner_{\bh^t})$ for the mixture in \eqref{eq:this}. We require these spanner policies instead of policies in the policy cover (as in \eqref{eq:this}) because the estimation of the $ Q$-functions becomes much more challenging with an adaptive adversary. 

%Following exploration, the algorithm proceeds in epochs. Each epoch (denoted as 'k') utilizes a fixed combination of policies:


%Exploitation Policy: Derived from an online learning algorithm, this policy is based on estimated Q-values from previous epochs. These Q-values function as loss functions, guiding the algorithm towards actions that are expected to maximize rewards.
%The combination of exploration and exploitation is crucial. Continuous exploration is needed to gather data and update the Q-values, ensuring the exploitation policy remains effective and adaptable as the algorithm learns.

==> widebar.tex <==
% Implementation of better \overline alternative from
% https://tex.stackexchange.com/questions/16337/can-i-get-a-widebar-without-using-the-mathabx-package.
% DF Note (8/15/20): Added underbar variant. Exactly the same except
% that \overline is replaced by \underline

%\usepackage{amsmath}
\makeatletter
\let\save@mathaccent\mathaccent
\newcommand*\if@single[3]{%
  \setbox0\hbox{${\mathaccent"0362{#1}}^H$}%
  \setbox2\hbox{${\mathaccent"0362{\kern0pt#1}}^H$}%
  \ifdim\ht0=\ht2 #3\else #2\fi
  }
%The bar will be moved to the right by a half of \macc@kerna, which is computed by amsmath:
\newcommand*\rel@kern[1]{\kern#1\dimexpr\macc@kerna}
%If there's a superscript following the bar, then no negative kern may follow the bar;
%an additional {} makes sure that the superscript is high enough in this case:
\newcommand*\widebar[1]{\@ifnextchar^{{\wide@bar{#1}{0}}}{\wide@bar{#1}{1}}}
%\newcommand*\underbar[1]{\@ifnextchar_{{\under@bar{#1}{0}}}{\under@bar{#1}{1}}}
%Use a separate algorithm for single symbols:
\newcommand*\wide@bar[2]{\if@single{#1}{\wide@bar@{#1}{#2}{1}}{\wide@bar@{#1}{#2}{2}}}
\newcommand*\under@bar[2]{\if@single{#1}{\under@bar@{#1}{#2}{1}}{\under@bar@{#1}{#2}{2}}}
\newcommand*\wide@bar@[3]{%
  \begingroup
  \def\mathaccent##1##2{%
%Enable nesting of accents:
    \let\mathaccent\save@mathaccent
%If there's more than a single symbol, use the first character instead (see below):
    \if#32 \let\macc@nucleus\first@char \fi
%Determine the italic correction:
    \setbox\z@\hbox{$\macc@style{\macc@nucleus}_{}$}%
    \setbox\tw@\hbox{$\macc@style{\macc@nucleus}{}_{}$}%
    \dimen@\wd\tw@
    \advance\dimen@-\wd\z@
%Now \dimen@ is the italic correction of the symbol.
    \divide\dimen@ 3
    \@tempdima\wd\tw@
    \advance\@tempdima-\scriptspace
%Now \@tempdima is the width of the symbol.
    \divide\@tempdima 10
    \advance\dimen@-\@tempdima
%Now \dimen@ = (italic correction / 3) - (Breite / 10)
    \ifdim\dimen@>\z@ \dimen@0pt\fi
%The bar will be shortened in the case \dimen@<0 !
    \rel@kern{0.6}\kern-\dimen@
    \if#31
      \overline{\rel@kern{-0.6}\kern\dimen@\macc@nucleus\rel@kern{0.4}\kern\dimen@}%
      \advance\dimen@0.4\dimexpr\macc@kerna
%Place the combined final kern (-\dimen@) if it is >0 or if a superscript follows:
      \let\final@kern#2%
      \ifdim\dimen@<\z@ \let\final@kern1\fi
      \if\final@kern1 \kern-\dimen@\fi
    \else
      \overline{\rel@kern{-0.6}\kern\dimen@#1}%
    \fi
  }%
  \macc@depth\@ne
  \let\math@bgroup\@empty \let\math@egroup\macc@set@skewchar
  \mathsurround\z@ \frozen@everymath{\mathgroup\macc@group\relax}%
  \macc@set@skewchar\relax
  \let\mathaccentV\macc@nested@a
%The following initialises \macc@kerna and calls \mathaccent:
  \if#31
    \macc@nested@a\relax111{#1}%
  \else
%If the argument consists of more than one symbol, and if the first token is
%a letter, use that letter for the computations:
    \def\gobble@till@marker##1\endmarker{}%
    \futurelet\first@char\gobble@till@marker#1\endmarker
    \ifcat\noexpand\first@char A\else
      \def\first@char{}%
    \fi
    \macc@nested@a\relax111{\first@char}%
  \fi
  \endgroup
}
\newcommand*\under@bar@[3]{%
  \begingroup
  \def\mathaccent##1##2{%
%Enable nesting of accents:
    \let\mathaccent\save@mathaccent
%If there's more than a single symbol, use the first character instead (see below):
    \if#32 \let\macc@nucleus\first@char \fi
%Determine the italic correction:
    \setbox\z@\hbox{$\macc@style{\macc@nucleus}_{}$}%
    \setbox\tw@\hbox{$\macc@style{\macc@nucleus}{}_{}$}%
    \dimen@\wd\tw@
    \advance\dimen@-\wd\z@
%Now \dimen@ is the italic correction of the symbol.
    \divide\dimen@ 3
    \@tempdima\wd\tw@
    \advance\@tempdima-\scriptspace
%Now \@tempdima is the width of the symbol.
    \divide\@tempdima 10
    \advance\dimen@-\@tempdima
%Now \dimen@ = (italic correction / 3) - (Breite / 10)
    \ifdim\dimen@>\z@ \dimen@0pt\fi
%The bar will be shortened in the case \dimen@<0 !
    \rel@kern{0.6}\kern-\dimen@
    \if#31
      \underline{\rel@kern{-0.6}\kern\dimen@\macc@nucleus\rel@kern{0.4}\kern\dimen@}%
      \advance\dimen@0.4\dimexpr\macc@kerna
%Place the combined final kern (-\dimen@) if it is >0 or if a superscript follows:
      \let\final@kern#2%
      \ifdim\dimen@<\z@ \let\final@kern1\fi
      \if\final@kern1 \kern-\dimen@\fi
    \else
      \underline{\rel@kern{-0.6}\kern\dimen@#1}%
    \fi
  }%
  \macc@depth\@ne
  \let\math@bgroup\@empty \let\math@egroup\macc@set@skewchar
  \mathsurround\z@ \frozen@everymath{\mathgroup\macc@group\relax}%
  \macc@set@skewchar\relax
  \let\mathaccentV\macc@nested@a
%The following initialises \macc@kerna and calls \mathaccent:
  \if#31
    \macc@nested@a\relax111{#1}%
  \else
%If the argument consists of more than one symbol, and if the first token is
%a letter, use that letter for the computations:
    \def\gobble@till@marker##1\endmarker{}%
    \futurelet\first@char\gobble@till@marker#1\endmarker
    \ifcat\noexpand\first@char A\else
      \def\first@char{}%
    \fi
    \macc@nested@a\relax111{\first@char}%
  \fi
  \endgroup
}
\makeatother


